The Relationship of Active Galactic Nuclei & Quasars With Their Local Galaxy Environment

We explore how the local environment is related to properties of active galactic nuclei (AGNs) of various luminosities. Recent simulations and observations are converging on the view that the extreme luminosity of quasars, the brightest of AGNs, is fueled in major mergers of gas-rich galaxies. In such a picture, quasars, the highest luminosity AGNs, are expected to be located in regions with a higher density of galaxies on small scales where mergers are more likely to take place. However, in this picture, the activity observed in low-luminosity AGNs is due to secular processes that are less dependent on the local galaxy density. To test this hypothesis, we compare the local photometric galaxy density on kiloparsec scales around spectroscopic type I and type II quasars to the local density around lower-luminosity spectroscopic type I and type II AGNs. To minimize projection effects and evolution in the photometric galaxy sample we use to characterize AGN environments, we place our random control sample at the same redshift as our AGNs and impose a narrow redshift window around both the AGNs and control targets. Our results support these merger models for bright AGN origins. We find that the brightest sources have overdensities that increase on the smallest scales compared to dimmer sources. In addition, we investigate the nature of the quasar and AGN environments themselves and find that the increased overdensity of early-type galaxies in the environments of bright type I sources suggests that they are located in richer cluster environments than dim sources. We measure increased environment overdensity with increased quasar black hole mass, consistent with the well-known M_{DMH}-M_{BH} relationship, and find evidence for quenching in the environments of high accretion efficiency type I quasars.

==> bibliography.tex <==
 \begin{thebibliography}{}

\bibitem[Abazajian et al.(2005)]{Abazajian} Abazajian, K., et al. \aj. 126.  2081.  2005. 
%\bibitem[Bevington(1969)]{Bevington}  Bevington, P. R.  \emph{Data Reduction and Error Analysis for the Physical Sciences}.  New York: McGraw-Hill Book Company, 1969.  
\bibitem[Hall, et al.(2000)]{Hall} Hall, P. B., et al. \apjs. 141.  267.  2002.
\bibitem[Hatziminaoglou et al.(2000)]{Hatzi} Hatziminaoglou, E., et al.  \aap.  359.  9-17.  2000.
\bibitem[Hogg(2000)]{Hogg} Hogg, D. W.  astro-ph/9905116.  2000.  
\bibitem[Hopkins et al.(2004)]{Hopkins}  Hopkins, P. F.  et al. \aj.  128. 1112-1123.  2004.  
\bibitem[Lupton(1993)]{Lupton} Lupton, R. H.  \emph{Statistics in Theory and Practice}.  Princeton: Princeton Univ. Press, 1993.
\bibitem[Lupton, Gunn, \& Szalay(1999)]{LuptonGunnSzalay}  Lupton, R. H., Gunn, J. E., \& Szalay, A. S.  \aj.  118.  1406-1410.  1999.  
\bibitem[Pogson(1856)]{Pogson}  Pogson, N. R. \mnras. 17, 12. 1856.  
\bibitem[Richards et al.(2001a)]{RichardsA}  Richards, G. T. et al. \aj.  121.  2308-2330. 2001a.
\bibitem[Richards et al.(2001b)]{RichardsB}  Richards, G. T. et al. \aj.  122.  1151-1162.  2001b.
\bibitem[Richards et al.(2006)]{Richards06}  Richards, G. T. et al. \aj.  131.  2766-2787.  2006.  
\bibitem[Schneider et al.(2005)]{Schneider}  Schneider, D. P. et al. astro-ph/0503679.  2005.  
\bibitem[Scranton et al.(2005)]{Scranton}  Scranton, R. et al.  astro-ph/0508564.  2005.  
\bibitem[Weinstein(2002)]{WeinsteinThesis}  Weinstein, M. A.  \emph{Photometric Redshifts of Quasars (A Sloan Digital Sky Survey Project)}.  Diss. The Pennsylvania State University. 2002.  
\bibitem[Weinstein et al.(2004)]{Weinstein}  Weinstein, M. A. et al.  \apjs.  155.  243-256.  2004.  
\bibitem[Wisotzki(2000)]{Wisotzki} Wisotzki, L.  \aap. 353.  861-866.  2000.  

\end{thebibliography}


==> photozs_tablesfigures.tex <==
 \clearpage

\begin{figure}
\plotone{gmedian_corrdiff.pdf}
\caption{The difference between Gaussian median CZRs without and with inclusion of correlation between SDSS bands for the four SDSS colors.  \label{corrCZRcomparefigures_median}}
\end{figure}

\begin{figure}
\plotone{gmode_corrdiff.pdf}
\caption{The difference between Gaussian mode (right) CZRs without and with inclusion of correlation between SDSS bands for the four SDSS colors.  \label{corrCZRcomparefigures_mode}}
\end{figure}

\begin{figure}
\plotone{zspeczphot_withdivisions_lw6.pdf}
\caption{Photometric redshift estimates are plotted against SDSS spectroscopic redshift for recreation of W04 algorithm.  Catastrophic failures, where $|$$z_{spec}$ - $z_{phot}$$|$ $\geqslant$ 0.5, are shown in red.  Black points have $|$$z_{spec}$ - $z_{phot}$$|$ $<$ 0.5.  Divisions for the four catastrophic failure sections (in z$_{phot}$) are shown in blue. \label{zspeczphot_withdivisions}}
\end{figure}

\begin{figure}
\plotone{colorcolor_catastrophics.pdf}
\caption{Color-color plots for all catastrophic failures (red points) superimposed on the entire quasar sample (black points) \label{colorcolor_allCF}}
\end{figure}

\begin{figure}
\plotone{colorcolor_section1.pdf}
\caption{Color-color plots for quasars in catastrophic failure section 1 (red points). Since there are so few points in this section (144), the points have been enlarged for easy viewing.  Black points show all other quasars in the sample (including other catastrophic failures. \label{colorcolor_sec1CF}}
\end{figure}

\begin{figure}
\plotone{colorcolor_section2.pdf}
\caption{Color-color plots for quasars in catastrophic failure section 2 (red points). Black points show all other quasars in the sample (including other catastrophic failures. \label{colorcolor_sec2CF}}
\end{figure}

\begin{figure}
\plotone{colorcolor_section3.pdf}
\caption{Color-color plots for quasars in catastrophic failure section 3 (red points). Black points show all other quasars in the sample (including other catastrophic failures. \label{colorcolor_sec3CF}}
\end{figure}

\begin{figure}
\plotone{colorcolor_section4.pdf}
\caption{Color-color plots for quasars in catastrophic failure section 4 (red points). Black points show all other quasars in the sample (including other catastrophic failures. \label{colorcolor_sec4CF}}
\end{figure}

\clearpage
    \begin{deluxetable}{r | l}
    \tablecolumns{2}
    \tablehead{\colhead{Parameter}&\colhead{Possible Variations}}
    \tablecaption{Summary of CZR and Photometric Redshift Algorithm Variations \label{variationSummary}}
    \startdata
    Binning&\emph{overlapping}\\
    &non-overlapping\\
    \cline{1-2}
    Statistic&\emph{mean}\\
    &discrete median\\
    &Gaussian median\\
    &discrete mode\\
    &Gaussian mode\\
    \cline{1-2}
    SDSS Magnitude Type&\emph{PSF}\\
    &model\\
    &fiber\\
    &Petrosian\\
    &convolve PDFs for multiple magnitude types\\
    \cline{1-2}
    Treatment of Reddened Quasars&\emph{removed}\\
    &not removed\\
    &redefined(?)\\
    \cline{1-2}
    Error and Magnitude Limits&\emph{not explicity imposed}\\
    &impose magnitude limits\\
    &impose error limits\\
    &impose combination of limits\\
    \cline{1-2}
    PDF Weighting&no weight function\\
    &\emph{simple N(z)}\\
    &apparent magnitude N(m, z)\\
    &luminosity function\\
    \cline{1-2}
    Additional Bands&\\
    \enddata
    \tablecomments{The parameter variation used by W04 is shown in italics.}
    \end{deluxetable}

    \begin{deluxetable}{c c c c c c}
    \tablecolumns{6}
%    \rotate
   \tablehead{\colhead{Variation} & \colhead{width  \emph{z} $\leq$  division1 } & \colhead{division 1} & \colhead{width division1 $<$ \emph{z} $\leq$ division 2} & \colhead{division 2} & \colhead{width \emph{z} $>$ division2}}
    \tablecaption{Redshift binning schemes.  \label{binningtable}}
    \startdata
    A&        &0.0&0.05&2.1&0.2\\
    B&        &0.0&0.05&2.1&0.1\\
    C&        &0.0&0.05&2.25&0.2\\
    D&        &0.0&0.05&2.25&0.1\\
    E&0.05&0.1&0.025&2.25&0.2\\
    F&0.05&0.1&0.025&2.25&0.1\\
    G&0.05&0.1&0.0125&2.25&0.2\\
    H&0.05&0.1&0.0125&2.25&0.1\\
    \enddata
    \tablecomments{The (non-overlapping) bin schemes listed in the table above are based on what is referred to in this paper as the O2 (overlapping) binscheme.  This scheme is used by \citet{RichardsB} and \citet{Weinstein}:  bins are centered at intervals in redshift of 0.05; bins with centers \emph{z} $\leq$ 2.15 have width 0.075, bins with centers at 2.15 $<$ \emph{z} $\leq$ 2.5 have width 0.2, and bins with centers at \emph{z} $>$ 2.5 have width 0.5.}  
    \end{deluxetable}
    
    \begin{deluxetable}{c c}
    \tablecolumns{2}
    \tablehead{\colhead{Fitting Parameter} & \colhead{Value}}
    \tablecaption{Parameters for Luminosity Function. \label{LumFconstants}}
    \startdata
    A$_{1}$&0.78\\
    B$_{1}$&0.10\\
    B$_{2}$&27.35\\
    B$_{3}$&19.27\\
    M$^{*}$&-26\\
    z$_{ref}$&2.45\\
    log($\Phi^{*}$)&-5.75
    \enddata
    \tablecomments{The values of these parameters are from \citet{Richards06} using the "Fixed Power Law" form of the luminosity function they derived.  $\Phi^{*}$ has units Mpc$^{-3}$mag$^{-1}$}
    \end{deluxetable}
    
    \begin{deluxetable}{c c}
    \tablecolumns{2}
    \tablehead{\colhead{Bands} & \colhead{c$_{ij}$}}
    \tablecaption{Correlation coefficients between SDSS filter bands.  \label{corrcoefftable}}
    \startdata
    c$_{ug}$&0.3\\
    c$_{ur}$&0.2\\
    c$_{ui}$&0.1\\
    c$_{uz}$&0.05\\
    c$_{gr}$&0.3\\
    c$_{gi}$&0.2\\
    c$_{gz}$&0.05\\
    c$_{ri}$&0.3\\
    c$_{rz}$&0.05\\
    c$_{iz}$&0.05
    \enddata
    \tablecomments{The values in this table are estimated from Figure 7 in \citet{Scranton}}  
    \end{deluxetable}


    \begin{deluxetable}{c c c c c}
    \tablecolumns{5}
   \tablehead{\colhead{Section} & \colhead{Range} & \colhead{Number of CF objects} & \colhead{Number of BALQSOs} & \colhead{$\%$ of section}}
    \tablecaption{Catastrophic Failure Sections for Analysis.  \label{CFsectionstable}}
    \startdata
    1&z$_{phot}$ $>$ 4.0 and z$_{phot}$ $>$ z$_{spec}$&143&45&31.5\\
    2&2.4 $<$ z$_{phot}$ $<$ 4.0 and z$_{phot}$ $>$ z$_{spec}$&1078&396&36.7\\
    2a&2.4 $<$ z$_{phot}$ $<$ 4.0 and z$_{phot}$ $<$ z$_{spec}$&5&1&20.0\\
    3&z$_{phot} $$<$ 2.4 and z$_{phot} $$>$ z$_{spec}$&3374&586&17.4\\
    4&z$_{phot} $$< $2.4 and z$_{phot}$ $<$ z$_{spec}$&2221&1273&57.4
    \enddata
    \end{deluxetable}

\clearpage

     \begin{deluxetable}{c c c c c c || c c c c | c c | c c | c c | c }
     \rotate
     \tablecolumns{17}
     \tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{All} & \multicolumn{7}{c}{Catastrophic Failures} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$} & 
     \colhead{CF} & 
     \colhead{\% CF} & 
     \colhead{Common} & 
     \colhead{\%} &
     \colhead{Diff} & 
     \colhead{\%} & 
     \colhead{not CF}}
     \tablecaption{PDF Photometric Redshift Estimates using Simple Weighting Function and removing reddened quasars.  \label{PDFsimpleWFremovered_table}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3835&0.5889&0.7648&0.8232&6821&0.1469&NA&NA&NA&NA&NA\\
\cline{1-17}
PDF&psf&A&mean&yes&SimpleWF&0.3878&0.5933&0.7612&0.8192&6822&0.1470&5645&0.8275&693&0.1016&1176\\
PDF&psf&C&mean&yes&SimpleWF&0.3975&0.6072&0.7700&0.8258&6524&0.1405&5189&0.7954&875&0.1341&1632\\
PDF&psf&E&mean&yes&SimpleWF&0.3967&0.5983&0.7671&0.8265&6503&0.1401&5093&0.7832&942&0.1449&1728\\
PDF&psf&G&mean&yes&SimpleWF&0.3930&0.5905&0.7569&0.8175&6872&0.1480&4926&0.7168&1459&0.2123&1895\\
PDF&model&O2&mean&yes&SimpleWF&0.3940&0.5988&0.7697&0.8271&6690&0.1443&5533&0.8271&689&0.1030&1288\\
PDF&model&A&mean&yes&SimpleWF&0.3948&0.5978&0.7619&0.8179&6921&0.1493&5255&0.7593&1187&0.1715&1566\\
PDF&model&C&mean&yes&SimpleWF&0.4086&0.6151&0.7750&0.8290&6418&0.1384&4837&0.7537&1132&0.1764&1984\\
PDF&model&E&mean&yes&SimpleWF&0.4123&0.6104&0.7714&0.8305&6360&0.1372&4747&0.7464&1174&0.1846&2074\\
PDF&model&G&mean&yes&SimpleWF&0.4083&0.6007&0.7636&0.8238&6673&0.1439&4682&0.7016&1522&0.2281&2139\\
PDF&fiber&O2&mean&yes&SimpleWF&0.3753&0.5755&0.7533&0.8132&7228&0.1559&5074&0.7020&1622&0.2244&1747\\
PDF&fiber&A&mean&yes&SimpleWF&0.3752&0.5711&0.7363&0.7925&7973&0.1720&5006&0.6279&2386&0.2993&1815\\
PDF&fiber&C&mean&yes&SimpleWF&0.3908&0.5932&0.7583&0.8138&6935&0.1496&4660&0.6720&1767&0.2548&2161\\
PDF&fiber&E&mean&yes&SimpleWF&0.3941&0.5903&0.7555&0.8150&6878&0.1484&4594&0.6679&1782&0.2591&2227\\
PDF&fiber&G&mean&yes&SimpleWF&0.3859&0.5807&0.7494&0.8092&7160&0.1544&4474&0.6249&2156&0.3011&2347\\
PDF&petro&O2&mean&yes&SimpleWF&0.3159&0.5018&0.6883&0.7616&8701&0.1877&4659&0.5355&3453&0.3969&2162\\
PDF&petro&A&mean&yes&SimpleWF&0.3223&0.5082&0.6794&0.7476&9306&0.2007&4557&0.4897&4113&0.4420&2264\\
PDF&petro&C&mean&yes&SimpleWF&0.3351&0.5276&0.7005&0.7666&8449&0.1823&4200&0.4971&3678&0.4353&2621\\
PDF&petro&E&mean&yes&SimpleWF&0.3410&0.5244&0.6933&0.7656&8362&0.1804&4246&0.5078&3525&0.4215&2575\\
PDF&petro&G&mean&yes&SimpleWF&0.3307&0.5154&0.6866&0.7576&8810&0.1900&4244&0.4817&3958&0.4493&2577\\
\cline{1-17}
PDF&psf&O2&gmedian&yes&SimpleWF&0.3787&0.5840&0.7577&0.8193&6933&0.1494&6062&0.8744&382&0.0551&759\\
PDF&psf&A&gmedian&yes&SimpleWF&0.3857&0.5892&0.7576&0.8172&6856&0.1477&5636&0.8221&727&0.1060&1185\\
PDF&psf&C&gmedian&yes&SimpleWF&0.3950&0.6023&0.7661&0.8235&6600&0.1422&5247&0.7950&885&0.1341&1574\\
PDF&psf&E&gmedian&yes&SimpleWF&0.3958&0.5962&0.7632&0.8228&6634&0.1429&5127&0.7728&1038&0.1565&1694\\
PDF&psf&G&gmedian&yes&SimpleWF&0.3906&0.5879&0.7535&0.8149&6961&0.1500&4927&0.7078&1537&0.2208&1894\\
PDF&model&O2&gmedian&yes&SimpleWF&0.3871&0.5898&0.7592&0.8190&6944&0.1498&5495&0.7913&958&0.1380&1326\\
PDF&model&A&gmedian&yes&SimpleWF&0.3969&0.5991&0.7612&0.8184&6788&0.1464&5238&0.7717&1078&0.1588&1583\\
PDF&model&C&gmedian&yes&SimpleWF&0.4064&0.6107&0.7691&0.8246&6513&0.1405&4896&0.7517&1166&0.1790&1925\\
PDF&model&E&gmedian&yes&SimpleWF&0.4124&0.6079&0.7676&0.8264&6494&0.1401&4761&0.7331&1275&0.1963&2060\\
PDF&model&G&gmedian&yes&SimpleWF&0.4056&0.5979&0.7596&0.8202&6764&0.1459&4643&0.6864&1638&0.2422&2178\\
PDF&fiber&O2&gmedian&yes&SimpleWF&0.3750&0.5725&0.7491&0.8117&7235&0.1561&5108&0.7060&1603&0.2216&1713\\
PDF&fiber&A&gmedian&yes&SimpleWF&0.3750&0.5699&0.7357&0.7927&7866&0.1697&5013&0.6373&2276&0.2893&1808\\
PDF&fiber&C&gmedian&yes&SimpleWF&0.3881&0.5886&0.7537&0.8104&6990&0.1508&4695&0.6717&1780&0.2546&2126\\
PDF&fiber&E&gmedian&yes&SimpleWF&0.3920&0.5888&0.7518&0.8123&6934&0.1496&4610&0.6648&1811&0.2612&2211\\
PDF&fiber&G&gmedian&yes&SimpleWF&0.3860&0.5799&0.7464&0.8064&7214&0.1556&4485&0.6217&2193&0.3040&2336\\
PDF&petro&O2&gmedian&yes&SimpleWF&0.3134&0.4972&0.6815&0.7568&8842&0.1907&4696&0.5311&3538&0.4001&2125\\
PDF&petro&A&gmedian&yes&SimpleWF&0.3233&0.5083&0.6816&0.7506&9026&0.1947&4560&0.5052&3846&0.4261&2261\\
PDF&petro&C&gmedian&yes&SimpleWF&0.3280&0.5173&0.6920&0.7585&8717&0.1880&4305&0.4939&3825&0.4388&2516\\
PDF&petro&E&gmedian&yes&SimpleWF&0.3370&0.5192&0.6880&0.7604&8549&0.1844&4308&0.5039&3642&0.4260&2513\\
PDF&petro&G&gmedian&yes&SimpleWF&0.3297&0.5105&0.6824&0.7548&8884&0.1916&4294&0.4833&3972&0.4471&2527\\
\cline{1-17}
PDF&psf&O2&gmode&yes&SimpleWF&0.3675&0.5696&0.7451&0.8105&7224&0.1556&5795&0.8022&924&0.1279&1026\\
PDF&psf&A&gmode&yes&SimpleWF&0.3745&0.5743&0.7434&0.8058&7214&0.1554&5489&0.7609&1209&0.1676&1332\\
PDF&psf&C&gmode&yes&SimpleWF&0.3866&0.5924&0.7586&0.8181&6722&0.1448&5283&0.7859&955&0.1421&1538\\
PDF&psf&E&gmode&yes&SimpleWF&0.3831&0.5824&0.7526&0.8144&6984&0.1505&5113&0.7321&1374&0.1967&1708\\
PDF&psf&G&gmode&yes&SimpleWF&0.3725&0.5706&0.7428&0.8043&7388&0.1592&4933&0.6677&1920&0.2599&1888\\
PDF&model&O2&gmode&yes&SimpleWF&0.3743&0.5731&0.7436&0.8066&7379&0.1592&5361&0.7265&1500&0.2033&1460\\
PDF&model&A&gmode&yes&SimpleWF&0.3766&0.5734&0.7376&0.7977&7544&0.1627&5118&0.6784&1891&0.2507&1703\\
PDF&model&C&gmode&yes&SimpleWF&0.3916&0.5961&0.7598&0.8188&6664&0.1437&4917&0.7378&1262&0.1894&1904\\
PDF&model&E&gmode&yes&SimpleWF&0.3910&0.5894&0.7583&0.8190&6785&0.1464&4758&0.7013&1541&0.2271&2063\\
PDF&model&G&gmode&yes&SimpleWF&0.3766&0.5721&0.7434&0.8054&7353&0.1586&4662&0.6340&2163&0.2942&2159\\
PDF&fiber&O2&gmode&yes&SimpleWF&0.3589&0.5549&0.7329&0.7971&7696&0.1660&4971&0.6459&2173&0.2824&1850\\
PDF&fiber&A&gmode&yes&SimpleWF&0.3596&0.5570&0.7288&0.7927&7669&0.1654&4885&0.6370&2222&0.2897&1936\\
PDF&fiber&C&gmode&yes&SimpleWF&0.3650&0.5658&0.7373&0.7992&7432&0.1603&4716&0.6346&2162&0.2909&2105\\
PDF&fiber&E&gmode&yes&SimpleWF&0.3659&0.5635&0.7332&0.7967&7631&0.1646&4669&0.6118&2389&0.3131&2152\\
PDF&fiber&G&gmode&yes&SimpleWF&0.3515&0.5437&0.7213&0.7854&8194&0.1767&4584&0.5594&2999&0.3660&2237\\
PDF&petro&O2&gmode&yes&SimpleWF&0.3008&0.4788&0.6616&0.7450&9025&0.1947&4647&0.5149&3759&0.4165&2174\\
PDF&petro&A&gmode&yes&SimpleWF&0.3047&0.4852&0.6574&0.7342&9634&0.2078&4573&0.4747&4396&0.4563&2248\\
PDF&petro&C&gmode&yes&SimpleWF&0.3133&0.5010&0.6764&0.7510&8885&0.1917&4348&0.4894&3940&0.4434&2473\\
PDF&petro&E&gmode&yes&SimpleWF&0.3156&0.4964&0.6741&0.7497&8980&0.1937&4351&0.4845&4011&0.4467&2470\\
PDF&petro&G&gmode&yes&SimpleWF&0.2978&0.4776&0.6551&0.7296&9976&0.2152&4373&0.4384&4897&0.4909&2448
     \enddata
     \end{deluxetable}
     
     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for low-redshift quasars using Simple Weighting Function and removing reddened quasars.  \label{PDFsimpleWFremovered_lowtable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3947&0.6036&0.7689&0.8196\\
\cline{1-10}
PDF&psf&A&mean&yes&SimpleWF&0.4065&0.6063&0.7648&0.8155\\
PDF&psf&C&mean&yes&SimpleWF&0.4177&0.6222&0.7748&0.8215\\
PDF&psf&E&mean&yes&SimpleWF&0.4153&0.6076&0.7660&0.8165\\
PDF&psf&G&mean&yes&SimpleWF&0.4102&0.5969&0.7520&0.8039\\
PDF&model&O2&mean&yes&SimpleWF&0.4066&0.6152&0.7761&0.8252\\
PDF&model&A&mean&yes&SimpleWF&0.4148&0.6121&0.7667&0.8148\\
PDF&model&C&mean&yes&SimpleWF&0.4302&0.6314&0.7807&0.8250\\
PDF&model&E&mean&yes&SimpleWF&0.4331&0.6219&0.7712&0.8212\\
PDF&model&G&mean&yes&SimpleWF&0.4278&0.6090&0.7603&0.8112\\
PDF&fiber&O2&mean&yes&SimpleWF&0.3891&0.5935&0.7588&0.8086\\
PDF&fiber&A&mean&yes&SimpleWF&0.3911&0.5809&0.7369&0.7868\\
PDF&fiber&C&mean&yes&SimpleWF&0.4097&0.6055&0.7610&0.8081\\
PDF&fiber&E&mean&yes&SimpleWF&0.4119&0.5982&0.7523&0.8032\\
PDF&fiber&G&mean&yes&SimpleWF&0.4018&0.5855&0.7432&0.7942\\
PDF&petro&O2&mean&yes&SimpleWF&0.3275&0.5184&0.6956&0.7586\\
PDF&petro&A&mean&yes&SimpleWF&0.3351&0.5180&0.6839&0.7439\\
PDF&petro&C&mean&yes&SimpleWF&0.3498&0.5377&0.7043&0.7626\\
PDF&petro&E&mean&yes&SimpleWF&0.3547&0.5286&0.6885&0.7532\\
PDF&petro&G&mean&yes&SimpleWF&0.3418&0.5155&0.6773&0.7400\\
\cline{1-10}
PDF&psf&O2&gmedian&yes&SimpleWF&0.3899&0.5982&0.7614&0.8157\\
PDF&psf&A&gmedian&yes&SimpleWF&0.4043&0.6019&0.7610&0.8136\\
PDF&psf&C&gmedian&yes&SimpleWF&0.4147&0.6160&0.7694&0.8184\\
PDF&psf&E&gmedian&yes&SimpleWF&0.4141&0.6048&0.7609&0.8120\\
PDF&psf&G&gmedian&yes&SimpleWF&0.4075&0.5937&0.7479&0.8009\\
PDF&model&O2&gmedian&yes&SimpleWF&0.3989&0.6045&0.7646&0.8167\\
PDF&model&A&gmedian&yes&SimpleWF&0.4172&0.6137&0.7660&0.8156\\
PDF&model&C&gmedian&yes&SimpleWF&0.4277&0.6263&0.7736&0.8198\\
PDF&model&E&gmedian&yes&SimpleWF&0.4333&0.6192&0.7670&0.8166\\
PDF&model&G&gmedian&yes&SimpleWF&0.4248&0.6060&0.7555&0.8072\\
PDF&fiber&O2&gmedian&yes&SimpleWF&0.3884&0.5884&0.7533&0.8068\\
PDF&fiber&A&gmedian&yes&SimpleWF&0.3913&0.5802&0.7366&0.7875\\
PDF&fiber&C&gmedian&yes&SimpleWF&0.4070&0.6004&0.7559&0.8041\\
PDF&fiber&E&gmedian&yes&SimpleWF&0.4101&0.5968&0.7487&0.8005\\
PDF&fiber&G&gmedian&yes&SimpleWF&0.4025&0.5851&0.7404&0.7916\\
PDF&petro&O2&gmedian&yes&SimpleWF&0.3249&0.5126&0.6879&0.7543\\
PDF&petro&A&gmedian&yes&SimpleWF&0.3378&0.5210&0.6894&0.7498\\
PDF&petro&C&gmedian&yes&SimpleWF&0.3418&0.5262&0.6940&0.7526\\
PDF&petro&E&gmedian&yes&SimpleWF&0.3504&0.5231&0.6822&0.7468\\
PDF&petro&G&gmedian&yes&SimpleWF&0.3410&0.5104&0.6723&0.7364\\
\cline{1-10}
PDF&psf&O2&gmode&yes&SimpleWF&0.3745&0.5808&0.7469&0.8026\\
PDF&psf&A&gmode&yes&SimpleWF&0.3910&0.5852&0.7435&0.7975\\
PDF&psf&C&gmode&yes&SimpleWF&0.4045&0.6035&0.7589&0.8094\\
PDF&psf&E&gmode&yes&SimpleWF&0.3995&0.5893&0.7492&0.8023\\
PDF&psf&G&gmode&yes&SimpleWF&0.3869&0.5746&0.7363&0.7890\\
PDF&model&O2&gmode&yes&SimpleWF&0.3838&0.5868&0.7460&0.7988\\
PDF&model&A&gmode&yes&SimpleWF&0.3932&0.5846&0.7381&0.7890\\
PDF&model&C&gmode&yes&SimpleWF&0.4104&0.6078&0.7606&0.8100\\
PDF&model&E&gmode&yes&SimpleWF&0.4091&0.5974&0.7556&0.8069\\
PDF&model&G&gmode&yes&SimpleWF&0.3921&0.5769&0.7377&0.7901\\
PDF&fiber&O2&gmode&yes&SimpleWF&0.3686&0.5680&0.7327&0.7868\\
PDF&fiber&A&gmode&yes&SimpleWF&0.3748&0.5677&0.7297&0.7859\\
PDF&fiber&C&gmode&yes&SimpleWF&0.3806&0.5737&0.7356&0.7890\\
PDF&fiber&E&gmode&yes&SimpleWF&0.3809&0.5686&0.7278&0.7826\\
PDF&fiber&G&gmode&yes&SimpleWF&0.3638&0.5448&0.7128&0.7683\\
PDF&petro&O2&gmode&yes&SimpleWF&0.3074&0.4884&0.6619&0.7366\\
PDF&petro&A&gmode&yes&SimpleWF&0.3137&0.4909&0.6572&0.7266\\
PDF&petro&C&gmode&yes&SimpleWF&0.3239&0.5043&0.6722&0.7403\\
PDF&petro&E&gmode&yes&SimpleWF&0.3251&0.4951&0.6643&0.7331\\
PDF&petro&G&gmode&yes&SimpleWF&0.3038&0.4718&0.6405&0.7076
     \enddata
     \end{deluxetable}
     
     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for high-redshift quasars using Simple Weighting Function and removing reddened quasars.  \label{PDFsimpleWFremovered_hightable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3303&0.5189&0.7458&0.8403\\
\cline{1-10}
PDF&psf&A&mean&yes&SimpleWF&0.2990&0.5318&0.7438&0.8369\\
PDF&psf&C&mean&yes&SimpleWF&0.2642&0.5079&0.7382&0.8544\\
PDF&psf&E&mean&yes&SimpleWF&0.2740&0.5368&0.7741&0.8927\\
PDF&psf&G&mean&yes&SimpleWF&0.2791&0.5482&0.7887&0.9076\\
PDF&model&O2&mean&yes&SimpleWF&0.3343&0.5208&0.7389&0.8359\\
PDF&model&A&mean&yes&SimpleWF&0.3000&0.5295&0.7388&0.8327\\
PDF&model&C&mean&yes&SimpleWF&0.2656&0.5075&0.7373&0.8553\\
PDF&model&E&mean&yes&SimpleWF&0.2743&0.5349&0.7723&0.8925\\
PDF&model&G&mean&yes&SimpleWF&0.2792&0.5454&0.7856&0.9066\\
PDF&fiber&O2&mean&yes&SimpleWF&0.3098&0.4901&0.7272&0.8348\\
PDF&fiber&A&mean&yes&SimpleWF&0.2998&0.5243&0.7334&0.8199\\
PDF&fiber&C&mean&yes&SimpleWF&0.2656&0.5117&0.7400&0.8516\\
PDF&fiber&E&mean&yes&SimpleWF&0.2765&0.5387&0.7768&0.8932\\
PDF&fiber&G&mean&yes&SimpleWF&0.2808&0.5488&0.7909&0.9083\\
PDF&petro&O2&mean&yes&SimpleWF&0.2605&0.4233&0.6536&0.7760\\
PDF&petro&A&mean&yes&SimpleWF&0.2611&0.4619&0.6582&0.7653\\
PDF&petro&C&mean&yes&SimpleWF&0.2379&0.4613&0.6759&0.7931\\
PDF&petro&E&mean&yes&SimpleWF&0.2510&0.4961&0.7245&0.8476\\
PDF&petro&G&mean&yes&SimpleWF&0.2576&0.5149&0.7480&0.8741\\
\cline{1-10}
PDF&psf&O2&gmedian&yes&SimpleWF&0.3255&0.5165&0.7399&0.8367\\
PDF&psf&A&gmedian&yes&SimpleWF&0.2974&0.5286&0.7412&0.8345\\
PDF&psf&C&gmedian&yes&SimpleWF&0.2652&0.5115&0.7441&0.8575\\
PDF&psf&E&gmedian&yes&SimpleWF&0.2752&0.5397&0.7785&0.8939\\
PDF&psf&G&gmedian&yes&SimpleWF&0.2796&0.5495&0.7910&0.9071\\
PDF&model&O2&gmedian&yes&SimpleWF&0.3310&0.5204&0.7337&0.8301\\
PDF&model&A&gmedian&yes&SimpleWF&0.3001&0.5300&0.7383&0.8318\\
PDF&model&C&gmedian&yes&SimpleWF&0.2661&0.5078&0.7393&0.8561\\
PDF&model&E&gmedian&yes&SimpleWF&0.2743&0.5331&0.7718&0.8907\\
PDF&model&G&gmedian&yes&SimpleWF&0.2786&0.5445&0.7867&0.9066\\
PDF&fiber&O2&gmedian&yes&SimpleWF&0.3113&0.4965&0.7291&0.8348\\
PDF&fiber&A&gmedian&yes&SimpleWF&0.2978&0.5212&0.7315&0.8172\\
PDF&fiber&C&gmedian&yes&SimpleWF&0.2631&0.5106&0.7390&0.8523\\
PDF&fiber&E&gmedian&yes&SimpleWF&0.2724&0.5359&0.7727&0.8900\\
PDF&fiber&G&gmedian&yes&SimpleWF&0.2765&0.5454&0.7861&0.9045\\
PDF&petro&O2&gmedian&yes&SimpleWF&0.2590&0.4235&0.6510&0.7689\\
PDF&petro&A&gmedian&yes&SimpleWF&0.2548&0.4479&0.6446&0.7544\\
PDF&petro&C&gmedian&yes&SimpleWF&0.2364&0.4589&0.6790&0.7972\\
PDF&petro&E&gmedian&yes&SimpleWF&0.2484&0.4930&0.7260&0.8501\\
PDF&petro&G&gmedian&yes&SimpleWF&0.2553&0.5114&0.7496&0.8764\\
\cline{1-10}
PDF&psf&O2&gmode&yes&SimpleWF&0.3342&0.5167&0.7367&0.8482\\
PDF&psf&A&gmode&yes&SimpleWF&0.2961&0.5226&0.7427&0.8451\\
PDF&psf&C&gmode&yes&SimpleWF&0.2685&0.5188&0.7571&0.8750\\
PDF&psf&E&gmode&yes&SimpleWF&0.2750&0.5368&0.7753&0.8943\\
PDF&psf&G&gmode&yes&SimpleWF&0.2778&0.5443&0.7854&0.9060\\
PDF&model&O2&gmode&yes&SimpleWF&0.3292&0.5081&0.7321&0.8435\\
PDF&model&A&gmode&yes&SimpleWF&0.2980&0.5204&0.7353&0.8389\\
PDF&model&C&gmode&yes&SimpleWF&0.2676&0.5183&0.7547&0.8774\\
PDF&model&E&gmode&yes&SimpleWF&0.2717&0.5368&0.7760&0.8989\\
PDF&model&G&gmode&yes&SimpleWF&0.2738&0.5408&0.7816&0.9062\\
PDF&fiber&O2&gmode&yes&SimpleWF&0.3127&0.4928&0.7335&0.8461\\
PDF&fiber&A&gmode&yes&SimpleWF&0.2872&0.5065&0.7244&0.8250\\
PDF&fiber&C&gmode&yes&SimpleWF&0.2621&0.5135&0.7482&0.8661\\
PDF&fiber&E&gmode&yes&SimpleWF&0.2669&0.5304&0.7694&0.8897\\
PDF&fiber&G&gmode&yes&SimpleWF&0.2701&0.5364&0.7770&0.8986\\
PDF&petro&O2&gmode&yes&SimpleWF&0.2691&0.4331&0.6602&0.7850\\
PDF&petro&A&gmode&yes&SimpleWF&0.2616&0.4580&0.6582&0.7703\\
PDF&petro&C&gmode&yes&SimpleWF&0.2431&0.4791&0.7045&0.8219\\
PDF&petro&E&gmode&yes&SimpleWF&0.2533&0.5050&0.7383&0.8595\\
PDF&petro&G&gmode&yes&SimpleWF&0.2578&0.5157&0.7513&0.8746
     \enddata
     \end{deluxetable}     
          
\clearpage          
          
     \begin{deluxetable}{c c c c c c || c c c c | c c | c c | c c | c }
     \rotate
     \tablecolumns{17}
     \tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{All} & \multicolumn{7}{c}{Catastrophic Failures} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$} & 
     \colhead{CF} & 
     \colhead{\% CF} & 
     \colhead{Common} & 
     \colhead{\%} &
     \colhead{Diff} & 
     \colhead{\%} & 
     \colhead{not CF}}
     \tablecaption{PDF Photometric Redshift Estimates using Simple Weighting Function, without removing reddened quasars.  \label{PDFsimpleWFnoremovered_table}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3835&0.5889&0.7648&0.8232&6821&0.1469&NA&NA&NA&NA&NA\\
\cline{1-17}
PDF&psf&O2&mean&no&SimpleWF&0.3648&0.5736&0.7660&0.8242&6800&0.1465&4883&0.7181&1446&0.2126&1938\\
PDF&psf&A&mean&no&SimpleWF&0.3596&0.5638&0.7580&0.8198&6815&0.1468&4905&0.7197&1445&0.2120&1916\\
PDF&psf&C&mean&no&SimpleWF&0.3669&0.5737&0.7593&0.8168&6959&0.1499&4195&0.6028&2303&0.3309&2626\\
PDF&psf&E&mean&no&SimpleWF&0.3736&0.5799&0.7683&0.8284&6372&0.1373&4354&0.6833&1565&0.2456&2467\\
PDF&psf&G&mean&no&SimpleWF&0.3828&0.5890&0.7667&0.8274&6410&0.1381&4445&0.6934&1518&0.2368&2376\\
PDF&model&O2&mean&no&SimpleWF&0.3703&0.5769&0.7687&0.8269&6729&0.1451&4748&0.7056&1531&0.2275&2073\\
PDF&model&A&mean&no&SimpleWF&0.3624&0.5640&0.7548&0.8164&7010&0.1512&4737&0.6757&1813&0.2586&2084\\
PDF&model&C&mean&no&SimpleWF&0.3729&0.5776&0.7604&0.8174&6982&0.1506&4108&0.5884&2408&0.3449&2713\\
PDF&model&E&mean&no&SimpleWF&0.3807&0.5844&0.7693&0.8298&6389&0.1378&4195&0.6566&1758&0.2752&2626\\
PDF&model&G&mean&no&SimpleWF&0.3956&0.5982&0.7722&0.8332&6199&0.1337&4221&0.6809&1553&0.2505&2600\\
PDF&fiber&O2&mean&no&SimpleWF&0.3585&0.5622&0.7570&0.8180&7067&0.1524&4568&0.6464&2007&0.2840&2253\\
PDF&fiber&A&mean&no&SimpleWF&0.3487&0.5453&0.7332&0.7955&7862&0.1696&4578&0.5823&2731&0.3474&2243\\
PDF&fiber&C&mean&no&SimpleWF&0.3653&0.5681&0.7518&0.8095&7246&0.1563&4019&0.5547&2720&0.3754&2802\\
PDF&fiber&E&mean&no&SimpleWF&0.3727&0.5765&0.7585&0.8190&6696&0.1444&4109&0.6136&2118&0.3163&2712\\
PDF&fiber&G&mean&no&SimpleWF&0.3765&0.5797&0.7564&0.8182&6747&0.1455&4082&0.6050&2187&0.3241&2739\\
PDF&petro&O2&mean&no&SimpleWF&0.2777&0.4594&0.6645&0.7455&9272&0.2000&4388&0.4733&4272&0.4607&2433\\
PDF&petro&A&mean&no&SimpleWF&0.2812&0.4628&0.6573&0.7366&9569&0.2064&4410&0.4609&4518&0.4721&2411\\
PDF&petro&C&mean&no&SimpleWF&0.2956&0.4846&0.6749&0.7483&9094&0.1962&3963&0.4358&4532&0.4984&2858\\
PDF&petro&E&mean&no&SimpleWF&0.3089&0.4958&0.6819&0.7562&8709&0.1879&4010&0.4604&4098&0.4705&2811\\
PDF&petro&G&mean&no&SimpleWF&0.3187&0.5105&0.6902&0.7616&8450&0.1823&4015&0.4751&3857&0.4564&2806\\
\cline{1-17}
PDF&psf&O2&gmedian&no&SimpleWF&0.3633&0.5702&0.7601&0.8212&6917&0.1490&4854&0.7017&1580&0.2284&1967\\
PDF&psf&A&gmedian&no&SimpleWF&0.3580&0.5593&0.7518&0.8164&6897&0.1486&4841&0.7019&1585&0.2298&1980\\
PDF&psf&C&gmedian&no&SimpleWF&0.3646&0.5684&0.7545&0.8149&7003&0.1509&4214&0.6017&2315&0.3306&2607\\
PDF&psf&E&gmedian&no&SimpleWF&0.3730&0.5762&0.7635&0.8253&6516&0.1404&4382&0.6725&1679&0.2577&2439\\
PDF&psf&G&gmedian&no&SimpleWF&0.3816&0.5837&0.7613&0.8231&6558&0.1413&4439&0.6769&1670&0.2547&2382\\
PDF&model&O2&gmedian&no&SimpleWF&0.3684&0.5734&0.7616&0.8232&6859&0.1480&4737&0.6906&1665&0.2427&2084\\
PDF&model&A&gmedian&no&SimpleWF&0.3614&0.5626&0.7525&0.8153&6970&0.1503&4694&0.6735&1811&0.2598&2127\\
PDF&model&C&gmedian&no&SimpleWF&0.3686&0.5729&0.7555&0.8140&7090&0.1529&4145&0.5846&2474&0.3489&2676\\
PDF&model&E&gmedian&no&SimpleWF&0.3790&0.5811&0.7652&0.8275&6489&0.1400&4181&0.6443&1867&0.2877&2640\\
PDF&model&G&gmedian&no&SimpleWF&0.3933&0.5925&0.7660&0.8286&6374&0.1375&4198&0.6586&1738&0.2727&2623\\
PDF&fiber&O2&gmedian&no&SimpleWF&0.3570&0.5582&0.7514&0.8154&7131&0.1538&4581&0.6424&2044&0.2866&2240\\
PDF&fiber&A&gmedian&no&SimpleWF&0.3468&0.5439&0.7297&0.7930&7870&0.1698&4577&0.5816&2744&0.3487&2244\\
PDF&fiber&C&gmedian&no&SimpleWF&0.3613&0.5638&0.7460&0.8053&7344&0.1584&4087&0.5565&2754&0.3750&2734\\
PDF&fiber&E&gmedian&no&SimpleWF&0.3708&0.5714&0.7527&0.8157&6787&0.1464&4095&0.6034&2208&0.3253&2726\\
PDF&fiber&G&gmedian&no&SimpleWF&0.3728&0.5718&0.7488&0.8127&6891&0.1486&4100&0.5950&2305&0.3345&2721\\
PDF&petro&O2&gmedian&no&SimpleWF&0.2746&0.4547&0.6558&0.7383&9548&0.2060&4409&0.4618&4496&0.4709&2412\\
PDF&petro&A&gmedian&no&SimpleWF&0.2841&0.4666&0.6568&0.7374&9358&0.2019&4401&0.4703&4328&0.4625&2420\\
PDF&petro&C&gmedian&no&SimpleWF&0.2909&0.4777&0.6629&0.7380&9458&0.2040&4035&0.4266&4790&0.5064&2786\\
PDF&petro&E&gmedian&no&SimpleWF&0.3040&0.4860&0.6701&0.7476&8962&0.1933&4049&0.4518&4305&0.4804&2772\\
PDF&petro&G&gmedian&no&SimpleWF&0.3152&0.5034&0.6819&0.7557&8609&0.1857&4067&0.4724&3970&0.4611&2754\\
\cline{1-17}
PDF&psf&O2&gmode&no&SimpleWF&0.3546&0.5597&0.7510&0.8184&6890&0.1484&4821&0.6997&1576&0.2287&2000\\
PDF&psf&A&gmode&no&SimpleWF&0.3502&0.5502&0.7391&0.8070&7138&0.1538&4775&0.6690&1871&0.2621&2046\\
PDF&psf&C&gmode&no&SimpleWF&0.3607&0.5655&0.7507&0.8138&6901&0.1487&4239&0.6143&2192&0.3176&2582\\
PDF&psf&E&gmode&no&SimpleWF&0.3646&0.5692&0.7538&0.8174&6765&0.1457&4343&0.6420&1947&0.2878&2478\\
PDF&psf&G&gmode&no&SimpleWF&0.3650&0.5673&0.7474&0.8117&6967&0.1501&4398&0.6313&2085&0.2993&2423\\
PDF&model&O2&gmode&no&SimpleWF&0.3492&0.5516&0.7409&0.8103&7222&0.1558&4765&0.6598&1972&0.2731&2056\\
PDF&model&A&gmode&no&SimpleWF&0.3438&0.5408&0.7306&0.7967&7639&0.1648&4615&0.6041&2498&0.3270&2206\\
PDF&model&C&gmode&no&SimpleWF&0.3593&0.5634&0.7503&0.8105&7153&0.1543&4204&0.5877&2460&0.3439&2617\\
PDF&model&E&gmode&no&SimpleWF&0.3624&0.5679&0.7577&0.8208&6777&0.1462&4204&0.6203&2109&0.3112&2617\\
PDF&model&G&gmode&no&SimpleWF&0.3681&0.5684&0.7516&0.8180&6765&0.1459&4232&0.6256&2052&0.3033&2589\\
PDF&fiber&O2&gmode&no&SimpleWF&0.3438&0.5461&0.7399&0.8073&7252&0.1564&4506&0.6213&2232&0.3078&2315\\
PDF&fiber&A&gmode&no&SimpleWF&0.3364&0.5358&0.7250&0.7948&7598&0.1639&4473&0.5887&2591&0.3410&2348\\
PDF&fiber&C&gmode&no&SimpleWF&0.3432&0.5480&0.7337&0.7980&7604&0.1640&4202&0.5526&2869&0.3773&2619\\
PDF&fiber&E&gmode&no&SimpleWF&0.3479&0.5486&0.7376&0.8032&7319&0.1579&4219&0.5764&2568&0.3509&2602\\
PDF&fiber&G&gmode&no&SimpleWF&0.3431&0.5409&0.7277&0.7929&7704&0.1662&4229&0.5489&2906&0.3772&2592\\
PDF&petro&O2&gmode&no&SimpleWF&0.2644&0.4449&0.6483&0.7365&9152&0.1974&4409&0.4818&4128&0.4510&2412\\
PDF&petro&A&gmode&no&SimpleWF&0.2724&0.4504&0.6418&0.7306&9511&0.2052&4368&0.4593&4505&0.4737&2453\\
PDF&petro&C&gmode&no&SimpleWF&0.2821&0.4675&0.6571&0.7401&9215&0.1988&4031&0.4374&4574&0.4964&2790\\
PDF&petro&E&gmode&no&SimpleWF&0.2907&0.4717&0.6612&0.7449&8851&0.1909&3993&0.4511&4255&0.4807&2828\\
PDF&petro&G&gmode&no&SimpleWF&0.2964&0.4796&0.6620&0.7402&9138&0.1971&4116&0.4504&4413&0.4829&2705
     \enddata
     \end{deluxetable}   
     
     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for low-redshift quasars using Simple Weighting Function without removing reddened quasars.  \label{PDFsimpleWFnoremovered_lowtable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3947&0.6036&0.7689&0.8196\\
\cline{1-10}
PDF&psf&O2&mean&no&SimpleWF&0.3808&0.5970&0.7830&0.8359\\
PDF&psf&A&mean&no&SimpleWF&0.3794&0.5823&0.7729&0.8284\\
PDF&psf&C&mean&no&SimpleWF&0.3852&0.5885&0.7696&0.8198\\
PDF&psf&E&mean&no&SimpleWF&0.3901&0.5895&0.7710&0.8229\\
PDF&psf&G&mean&no&SimpleWF&0.3993&0.5962&0.7646&0.8164\\
PDF&model&O2&mean&no&SimpleWF&0.3849&0.5992&0.7853&0.8383\\
PDF&model&A&mean&no&SimpleWF&0.3832&0.5824&0.7700&0.8252\\
PDF&model&C&mean&no&SimpleWF&0.3918&0.5928&0.7704&0.8201\\
PDF&model&E&mean&no&SimpleWF&0.3984&0.5951&0.7730&0.8253\\
PDF&model&G&mean&no&SimpleWF&0.4141&0.6072&0.7713&0.8237\\
PDF&fiber&O2&mean&no&SimpleWF&0.3731&0.5832&0.7703&0.8254\\
PDF&fiber&A&mean&no&SimpleWF&0.3664&0.5603&0.7439&0.7993\\
PDF&fiber&C&mean&no&SimpleWF&0.3831&0.5824&0.7605&0.8113\\
PDF&fiber&E&mean&no&SimpleWF&0.3886&0.5850&0.7587&0.8112\\
PDF&fiber&G&mean&no&SimpleWF&0.3920&0.5858&0.7524&0.8059\\
PDF&petro&O2&mean&no&SimpleWF&0.2884&0.4756&0.6790&0.7547\\
PDF&petro&A&mean&no&SimpleWF&0.2955&0.4784&0.6745&0.7467\\
PDF&petro&C&mean&no&SimpleWF&0.3088&0.4963&0.6856&0.7541\\
PDF&petro&E&mean&no&SimpleWF&0.3205&0.5018&0.6836&0.7514\\
PDF&petro&G&mean&no&SimpleWF&0.3299&0.5135&0.6860&0.7495\\
\cline{1-10}
PDF&psf&O2&gmedian&no&SimpleWF&0.3789&0.5912&0.7745&0.8309\\
PDF&psf&A&gmedian&no&SimpleWF&0.3772&0.5763&0.7648&0.8236\\
PDF&psf&C&gmedian&no&SimpleWF&0.3815&0.5810&0.7618&0.8158\\
PDF&psf&E&gmedian&no&SimpleWF&0.3887&0.5841&0.7636&0.8180\\
PDF&psf&G&gmedian&no&SimpleWF&0.3973&0.5892&0.7570&0.8108\\
PDF&model&O2&gmedian&no&SimpleWF&0.3836&0.5943&0.7761&0.8330\\
PDF&model&A&gmedian&no&SimpleWF&0.3813&0.5807&0.7668&0.8235\\
PDF&model&C&gmedian&no&SimpleWF&0.3861&0.5860&0.7626&0.8143\\
PDF&model&E&gmedian&no&SimpleWF&0.3955&0.5898&0.7660&0.8206\\
PDF&model&G&gmedian&no&SimpleWF&0.4108&0.5997&0.7627&0.8173\\
PDF&fiber&O2&gmedian&no&SimpleWF&0.3709&0.5756&0.7617&0.8208\\
PDF&fiber&A&gmedian&no&SimpleWF&0.3640&0.5580&0.7395&0.7961\\
PDF&fiber&C&gmedian&no&SimpleWF&0.3777&0.5759&0.7522&0.8049\\
PDF&fiber&E&gmedian&no&SimpleWF&0.3858&0.5778&0.7506&0.8061\\
PDF&fiber&G&gmedian&no&SimpleWF&0.3873&0.5759&0.7427&0.7990\\
PDF&petro&O2&gmedian&no&SimpleWF&0.2849&0.4700&0.6694&0.7480\\
PDF&petro&A&gmedian&no&SimpleWF&0.2985&0.4833&0.6738&0.7481\\
PDF&petro&C&gmedian&no&SimpleWF&0.3027&0.4878&0.6709&0.7416\\
PDF&petro&E&gmedian&no&SimpleWF&0.3139&0.4885&0.6670&0.7387\\
PDF&petro&G&gmedian&no&SimpleWF&0.3252&0.5041&0.6745&0.7411\\
\cline{1-10}
PDF&psf&O2&gmode&no&SimpleWF&0.3681&0.5788&0.7618&0.8207\\
PDF&psf&A&gmode&no&SimpleWF&0.3657&0.5627&0.7448&0.8049\\
PDF&psf&C&gmode&no&SimpleWF&0.3757&0.5754&0.7547&0.8107\\
PDF&psf&E&gmode&no&SimpleWF&0.3782&0.5752&0.7520&0.8081\\
PDF&psf&G&gmode&no&SimpleWF&0.3779&0.5703&0.7416&0.7977\\
PDF&model&O2&gmode&no&SimpleWF&0.3607&0.5686&0.7484&0.8103\\
PDF&model&A&gmode&no&SimpleWF&0.3597&0.5538&0.7383&0.7951\\
PDF&model&C&gmode&no&SimpleWF&0.3739&0.5722&0.7533&0.8062\\
PDF&model&E&gmode&no&SimpleWF&0.3756&0.5727&0.7554&0.8103\\
PDF&model&G&gmode&no&SimpleWF&0.3813&0.5715&0.7460&0.8047\\
PDF&fiber&O2&gmode&no&SimpleWF&0.3535&0.5583&0.7415&0.8012\\
PDF&fiber&A&gmode&no&SimpleWF&0.3513&0.5498&0.7328&0.7947\\
PDF&fiber&C&gmode&no&SimpleWF&0.3561&0.5556&0.7352&0.7930\\
PDF&fiber&E&gmode&no&SimpleWF&0.3593&0.5507&0.7320&0.7905\\
PDF&fiber&G&gmode&no&SimpleWF&0.3531&0.5405&0.7188&0.7765\\
PDF&petro&O2&gmode&no&SimpleWF&0.2732&0.4561&0.6557&0.7387\\
PDF&petro&A&gmode&no&SimpleWF&0.2821&0.4598&0.6503&0.7328\\
PDF&petro&C&gmode&no&SimpleWF&0.2910&0.4727&0.6586&0.7376\\
PDF&petro&E&gmode&no&SimpleWF&0.2975&0.4693&0.6521&0.7301\\
PDF&petro&G&gmode&no&SimpleWF&0.3032&0.4760&0.6500&0.7214
     \enddata
     \end{deluxetable}

     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for high-redshift quasars using Simple Weighting Function without removing reddened quasars.  \label{PDFsimpleWFnoremovered_hightable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3303&0.5189&0.7458&0.8403\\
\cline{1-10}
PDF&psf&O2&mean&no&SimpleWF&0.2887&0.4624&0.6848&0.7687\\
PDF&psf&A&mean&no&SimpleWF&0.2655&0.4758&0.6869&0.7790\\
PDF&psf&C&mean&no&SimpleWF&0.2462&0.4760&0.6907&0.7967\\
PDF&psf&E&mean&no&SimpleWF&0.2644&0.5170&0.7499&0.8650\\
PDF&psf&G&mean&no&SimpleWF&0.2744&0.5414&0.7807&0.8999\\
PDF&model&O2&mean&no&SimpleWF&0.3008&0.4711&0.6894&0.7730\\
PDF&model&A&mean&no&SimpleWF&0.2636&0.4763&0.6822&0.7749\\
PDF&model&C&mean&no&SimpleWF&0.2482&0.4773&0.6947&0.7997\\
PDF&model&E&mean&no&SimpleWF&0.2643&0.5140&0.7454&0.8600\\
PDF&model&G&mean&no&SimpleWF&0.2735&0.5385&0.7780&0.8965\\
PDF&fiber&O2&mean&no&SimpleWF&0.2892&0.4628&0.6934&0.7825\\
PDF&fiber&A&mean&no&SimpleWF&0.2648&0.4741&0.6821&0.7771\\
PDF&fiber&C&mean&no&SimpleWF&0.2478&0.4737&0.6942&0.7978\\
PDF&fiber&E&mean&no&SimpleWF&0.2678&0.5204&0.7571&0.8705\\
PDF&fiber&G&mean&no&SimpleWF&0.2738&0.5395&0.7830&0.8992\\
PDF&petro&O2&mean&no&SimpleWF&0.2268&0.3823&0.5957&0.7016\\
PDF&petro&A&mean&no&SimpleWF&0.2131&0.3883&0.5754&0.6886\\
PDF&petro&C&mean&no&SimpleWF&0.2088&0.4068&0.6038&0.7097\\
PDF&petro&E&mean&no&SimpleWF&0.2321&0.4562&0.6705&0.7884\\
PDF&petro&G&mean&no&SimpleWF&0.2443&0.4901&0.7181&0.8414\\
\cline{1-10}
PDF&psf&O2&gmedian&no&SimpleWF&0.2892&0.4704&0.6917&0.7750\\
PDF&psf&A&gmedian&no&SimpleWF&0.2670&0.4784&0.6900&0.7818\\
PDF&psf&C&gmedian&no&SimpleWF&0.2526&0.4855&0.7060&0.8088\\
PDF&psf&E&gmedian&no&SimpleWF&0.2690&0.5242&0.7625&0.8735\\
PDF&psf&G&gmedian&no&SimpleWF&0.2781&0.5469&0.7897&0.9047\\
PDF&model&O2&gmedian&no&SimpleWF&0.2962&0.4739&0.6927&0.7764\\
PDF&model&A&gmedian&no&SimpleWF&0.2668&0.4763&0.6849&0.7765\\
PDF&model&C&gmedian&no&SimpleWF&0.2532&0.4863&0.7086&0.8118\\
PDF&model&E&gmedian&no&SimpleWF&0.2697&0.5234&0.7600&0.8728\\
PDF&model&G&gmedian&no&SimpleWF&0.2778&0.5449&0.7879&0.9034\\
PDF&fiber&O2&gmedian&no&SimpleWF&0.2907&0.4755&0.7026&0.7898\\
PDF&fiber&A&gmedian&no&SimpleWF&0.2651&0.4769&0.6836&0.7784\\
PDF&fiber&C&gmedian&no&SimpleWF&0.2526&0.4838&0.7052&0.8085\\
PDF&fiber&E&gmedian&no&SimpleWF&0.2713&0.5293&0.7669&0.8785\\
PDF&fiber&G&gmedian&no&SimpleWF&0.2772&0.5449&0.7886&0.9033\\
PDF&petro&O2&gmedian&no&SimpleWF&0.2252&0.3819&0.5910&0.6922\\
PDF&petro&A&gmedian&no&SimpleWF&0.2155&0.3870&0.5762&0.6864\\
PDF&petro&C&gmedian&no&SimpleWF&0.2129&0.4108&0.6102&0.7142\\
PDF&petro&E&gmedian&no&SimpleWF&0.2385&0.4694&0.6904&0.8068\\
PDF&petro&G&gmedian&no&SimpleWF&0.2486&0.4988&0.7309&0.8519\\
\cline{1-10}
PDF&psf&O2&gmode&no&SimpleWF&0.2901&0.4691&0.6995&0.8072\\
PDF&psf&A&gmode&no&SimpleWF&0.2768&0.4911&0.7119&0.8171\\
PDF&psf&C&gmode&no&SimpleWF&0.2613&0.5002&0.7238&0.8339\\
PDF&psf&E&gmode&no&SimpleWF&0.2749&0.5299&0.7654&0.8786\\
PDF&psf&G&gmode&no&SimpleWF&0.2799&0.5471&0.7859&0.9038\\
PDF&model&O2&gmode&no&SimpleWF&0.2942&0.4706&0.7050&0.8101\\
PDF&model&A&gmode&no&SimpleWF&0.2681&0.4792&0.6941&0.8042\\
PDF&model&C&gmode&no&SimpleWF&0.2627&0.5055&0.7304&0.8386\\
PDF&model&E&gmode&no&SimpleWF&0.2756&0.5365&0.7734&0.8901\\
PDF&model&G&gmode&no&SimpleWF&0.2809&0.5478&0.7880&0.9057\\
PDF&fiber&O2&gmode&no&SimpleWF&0.2975&0.4880&0.7319&0.8364\\
PDF&fiber&A&gmode&no&SimpleWF&0.2651&0.4696&0.6881&0.7954\\
PDF&fiber&C&gmode&no&SimpleWF&0.2583&0.4978&0.7241&0.8310\\
PDF&fiber&E&gmode&no&SimpleWF&0.2726&0.5350&0.7745&0.8872\\
PDF&fiber&G&gmode&no&SimpleWF&0.2767&0.5436&0.7865&0.9014\\
PDF&petro&O2&gmode&no&SimpleWF&0.2230&0.3919&0.6127&0.7260\\
PDF&petro&A&gmode&no&SimpleWF&0.2266&0.4060&0.6017&0.7199\\
PDF&petro&C&gmode&no&SimpleWF&0.2233&0.4334&0.6469&0.7567\\
PDF&petro&E&gmode&no&SimpleWF&0.2458&0.4878&0.7211&0.8424\\
PDF&petro&G&gmode&no&SimpleWF&0.2515&0.5035&0.7411&0.8647
     \enddata
     \end{deluxetable}

\clearpage

     \begin{deluxetable}{c c c c c c || c c c c | c c | c c | c c | c }
     \rotate
     \tablecolumns{17}
     \tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{All} & \multicolumn{7}{c}{Catastrophic Failures} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$} & 
     \colhead{\# CF} & 
     \colhead{\% CF} & 
     \colhead{\# Common} & 
     \colhead{\%} &
     \colhead{\# Diff} & 
     \colhead{\%} & 
     \colhead{\# not CF}}
     \tablecaption{PDF Photometric Redshift Estimates using No Weighting Function and removing reddened quasars.  \label{PDFnoWFremovered_table}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3835&0.5889&0.7648&0.8232&6821&0.1469&NA&NA&NA&NA&NA\\
\cline{1-17}
PDF&psf&O2&mean&yes&NoWF&0.3871&0.5890&0.7502&0.8074&7481&0.1612&4831&0.6458&2650&0.3542&1990\\
PDF&psf&A&mean&yes&NoWF&0.3885&0.5888&0.7462&0.7988&7814&0.1683&4584&0.5866&3230&0.4134&2237\\
PDF&psf&C&mean&yes&NoWF&0.3908&0.5934&0.7481&0.8024&7607&0.1639&4961&0.6522&2646&0.3478&1860\\
PDF&psf&E&mean&yes&NoWF&0.3968&0.5905&0.7457&0.8015&7637&0.1645&4801&0.6286&2836&0.3714&2020\\
PDF&psf&G&mean&yes&NoWF&0.4030&0.5922&0.7435&0.8011&7690&0.1657&4706&0.6120&2984&0.3880&2115\\
PDF&model&O2&mean&yes&NoWF&0.3985&0.5981&0.7548&0.8100&7372&0.1590&4613&0.6257&2248&0.3049&2208\\
PDF&model&A&mean&yes&NoWF&0.3971&0.5968&0.7506&0.8023&7623&0.1644&4380&0.5746&2724&0.3573&2441\\
PDF&model&C&mean&yes&NoWF&0.4037&0.6072&0.7594&0.8135&7090&0.1529&4621&0.6518&1982&0.2795&2200\\
PDF&model&E&mean&yes&NoWF&0.4163&0.6071&0.7555&0.8131&7110&0.1534&4582&0.6444&2055&0.2890&2239\\
PDF&model&G&mean&yes&NoWF&0.4178&0.6066&0.7529&0.8111&7203&0.1554&4528&0.6286&2189&0.3039&2293\\
PDF&fiber&O2&mean&yes&NoWF&0.3751&0.5736&0.7397&0.7960&7879&0.1700&4279&0.5431&3047&0.3867&2542\\
PDF&fiber&A&mean&yes&NoWF&0.3710&0.5632&0.7200&0.7733&8856&0.1910&4276&0.4828&3949&0.4459&2545\\
PDF&fiber&C&mean&yes&NoWF&0.3832&0.5815&0.7383&0.7937&7927&0.1710&4510&0.5689&2852&0.3598&2311\\
PDF&fiber&E&mean&yes&NoWF&0.3942&0.5849&0.7344&0.7924&7955&0.1716&4444&0.5586&2954&0.3713&2377\\
PDF&fiber&G&mean&yes&NoWF&0.3966&0.5833&0.7358&0.7937&7869&0.1697&4321&0.5491&3010&0.3825&2500\\
PDF&petro&O2&mean&yes&NoWF&0.3184&0.5004&0.6753&0.7423&9619&0.2075&3916&0.4071&5064&0.5265&2905\\
PDF&petro&A&mean&yes&NoWF&0.3238&0.5031&0.6665&0.7290&10357&0.2234&3938&0.3802&5747&0.5549&2883\\
PDF&petro&C&mean&yes&NoWF&0.3308&0.5136&0.6771&0.7406&9778&0.2109&4004&0.4095&5158&0.5275&2817\\
PDF&petro&E&mean&yes&NoWF&0.3375&0.5135&0.6714&0.7403&9661&0.2084&4135&0.4280&4907&0.5079&2686\\
PDF&petro&G&mean&yes&NoWF&0.3370&0.5146&0.6710&0.7388&9796&0.2113&4040&0.4124&5130&0.5237&2781\\
\cline{1-17}
PDF&psf&O2&gmedian&yes&NoWF&0.3843&0.5848&0.7458&0.8045&7543&0.1625&4910&0.6509&2633&0.3491&1911\\
PDF&psf&A&gmedian&yes&NoWF&0.3864&0.5857&0.7439&0.7971&7841&0.1689&4650&0.5930&3191&0.4070&2171\\
PDF&psf&C&gmedian&yes&NoWF&0.3875&0.5889&0.7437&0.7994&7677&0.1654&4986&0.6495&2691&0.3505&1835\\
PDF&psf&E&gmedian&yes&NoWF&0.3957&0.5875&0.7413&0.7982&7740&0.1667&4834&0.6245&2906&0.3755&1987\\
PDF&psf&G&gmedian&yes&NoWF&0.4003&0.5904&0.7397&0.7977&7793&0.1679&4752&0.6098&3041&0.3902&2069\\
PDF&model&O2&gmedian&yes&NoWF&0.3919&0.5893&0.7457&0.8031&7578&0.1635&4681&0.6177&2362&0.3117&2140\\
PDF&model&A&gmedian&yes&NoWF&0.3985&0.5952&0.7516&0.8039&7462&0.1610&4414&0.5915&2530&0.3391&2407\\
PDF&model&C&gmedian&yes&NoWF&0.4011&0.5995&0.7536&0.8085&7222&0.1558&4667&0.6462&2051&0.2840&2154\\
PDF&model&E&gmedian&yes&NoWF&0.4139&0.6015&0.7508&0.8090&7256&0.1565&4611&0.6355&2154&0.2969&2210\\
PDF&model&G&gmedian&yes&NoWF&0.4154&0.6002&0.7474&0.8060&7363&0.1588&4535&0.6159&2322&0.3154&2286\\
PDF&fiber&O2&gmedian&yes&NoWF&0.3760&0.5734&0.7400&0.7970&7747&0.1671&4368&0.5638&2846&0.3674&2453\\
PDF&fiber&A&gmedian&yes&NoWF&0.3703&0.5611&0.7193&0.7732&8780&0.1894&4349&0.4953&3816&0.4346&2472\\
PDF&fiber&C&gmedian&yes&NoWF&0.3819&0.5774&0.7351&0.7911&7950&0.1715&4524&0.5691&2859&0.3596&2297\\
PDF&fiber&E&gmedian&yes&NoWF&0.3915&0.5817&0.7298&0.7880&8098&0.1747&4462&0.5510&3079&0.3802&2359\\
PDF&fiber&G&gmedian&yes&NoWF&0.3942&0.5806&0.7303&0.7889&8050&0.1736&4334&0.5384&3166&0.3933&2487\\
PDF&petro&O2&gmedian&yes&NoWF&0.3134&0.4934&0.6700&0.7375&9722&0.2097&3996&0.4110&5072&0.5217&2825\\
PDF&petro&A&gmedian&yes&NoWF&0.3259&0.5049&0.6703&0.7329&10072&0.2173&3954&0.3926&5461&0.5422&2867\\
PDF&petro&C&gmedian&yes&NoWF&0.3275&0.5081&0.6734&0.7371&9894&0.2134&4059&0.4102&5191&0.5247&2762\\
PDF&petro&E&gmedian&yes&NoWF&0.3347&0.5097&0.6657&0.7347&9930&0.2142&4207&0.4237&5074&0.5110&2614\\
PDF&petro&G&gmedian&yes&NoWF&0.3331&0.5076&0.6618&0.7293&10192&0.2199&4088&0.4011&5438&0.5336&2733\\
\cline{1-17}
PDF&psf&O2&gmode&yes&NoWF&0.3757&0.5715&0.7356&0.7989&7717&0.1662&4925&0.6382&2792&0.3618&1896\\
PDF&psf&A&gmode&yes&NoWF&0.3719&0.5702&0.7301&0.7848&8297&0.1787&4796&0.5780&3501&0.4220&2025\\
PDF&psf&C&gmode&yes&NoWF&0.3723&0.5712&0.7272&0.7849&8248&0.1777&5022&0.6089&3226&0.3911&1799\\
PDF&psf&E&gmode&yes&NoWF&0.3774&0.5687&0.7235&0.7816&8492&0.1829&4936&0.5813&3556&0.4187&1885\\
PDF&psf&G&gmode&yes&NoWF&0.3785&0.5664&0.7216&0.7830&8354&0.1800&4799&0.5745&3555&0.4255&2022\\
PDF&model&O2&gmode&yes&NoWF&0.3766&0.5751&0.7335&0.7931&7963&0.1718&4742&0.5955&3221&0.4045&2079\\
PDF&model&A&gmode&yes&NoWF&0.3825&0.5764&0.7351&0.7879&8056&0.1738&4659&0.5783&2838&0.3523&2162\\
PDF&model&C&gmode&yes&NoWF&0.3849&0.5821&0.7394&0.7968&7601&0.1640&4738&0.6233&2863&0.3767&2083\\
PDF&model&E&gmode&yes&NoWF&0.3939&0.5868&0.7403&0.8009&7557&0.1630&4542&0.6010&2497&0.3304&2279\\
PDF&model&G&gmode&yes&NoWF&0.3851&0.5721&0.7291&0.7912&7835&0.1690&4496&0.5738&2795&0.3567&2325\\
PDF&fiber&O2&gmode&yes&NoWF&0.3663&0.5610&0.7290&0.7890&7968&0.1719&4348&0.5457&3064&0.3845&2473\\
PDF&fiber&A&gmode&yes&NoWF&0.3607&0.5564&0.7189&0.7772&8380&0.1808&4375&0.5221&3434&0.4098&2446\\
PDF&fiber&C&gmode&yes&NoWF&0.3584&0.5535&0.7132&0.7724&8645&0.1865&4608&0.5330&3434&0.3972&2213\\
PDF&fiber&E&gmode&yes&NoWF&0.3649&0.5558&0.7123&0.7723&8767&0.1891&4503&0.5136&3647&0.4160&2318\\
PDF&fiber&G&gmode&yes&NoWF&0.3653&0.5560&0.7112&0.7736&8705&0.1878&4440&0.5101&3655&0.4199&2381\\
PDF&petro&O2&gmode&yes&NoWF&0.2969&0.4699&0.6387&0.7115&10667&0.2301&3906&0.3662&6049&0.5671&2915\\
PDF&petro&A&gmode&yes&NoWF&0.3156&0.4971&0.6624&0.7308&10054&0.2169&4010&0.3988&5392&0.5363&2811\\
PDF&petro&C&gmode&yes&NoWF&0.3161&0.4971&0.6620&0.7335&9927&0.2141&4142&0.4172&5141&0.5179&2679\\
PDF&petro&E&gmode&yes&NoWF&0.3168&0.4917&0.6531&0.7251&10217&0.2204&4259&0.4169&5286&0.5174&2562\\
PDF&petro&G&gmode&yes&NoWF&0.3116&0.4898&0.6535&0.7236&10334&0.2229&4255&0.4117&5395&0.5221&2566
     \enddata
     \end{deluxetable}
     
     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for low-redshift quasars using No Weighting Function and removing reddened quasars.  \label{PDFnoWFremovered_lowtable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3947&0.6036&0.7689&0.8196\\
\cline{1-10}
PDF&psf&O2&mean&yes&NoWF&0.4105&0.6142&0.7657&0.8173\\
PDF&psf&A&mean&yes&NoWF&0.4180&0.6196&0.7670&0.8151\\
PDF&psf&C&mean&yes&NoWF&0.4112&0.6096&0.7521&0.7973\\
PDF&psf&E&mean&yes&NoWF&0.4181&0.6072&0.7508&0.7974\\
PDF&psf&G&mean&yes&NoWF&0.4253&0.6102&0.7495&0.7983\\
PDF&model&O2&mean&yes&NoWF&0.4226&0.6245&0.7706&0.8204\\
PDF&model&A&mean&yes&NoWF&0.4271&0.6275&0.7712&0.8185\\
PDF&model&C&mean&yes&NoWF&0.4259&0.6249&0.7650&0.8099\\
PDF&model&E&mean&yes&NoWF&0.4403&0.6259&0.7617&0.8104\\
PDF&model&G&mean&yes&NoWF&0.4418&0.6263&0.7599&0.8091\\
PDF&fiber&O2&mean&yes&NoWF&0.4018&0.6028&0.7564&0.8070\\
PDF&fiber&A&mean&yes&NoWF&0.4012&0.5949&0.7420&0.7907\\
PDF&fiber&C&mean&yes&NoWF&0.4019&0.5949&0.7410&0.7881\\
PDF&fiber&E&mean&yes&NoWF&0.4145&0.5984&0.7357&0.7850\\
PDF&fiber&G&mean&yes&NoWF&0.4176&0.5985&0.7383&0.7869\\
PDF&petro&O2&mean&yes&NoWF&0.3440&0.5319&0.6983&0.7599\\
PDF&petro&A&mean&yes&NoWF&0.3533&0.5375&0.6960&0.7528\\
PDF&petro&C&mean&yes&NoWF&0.3471&0.5264&0.6800&0.7347\\
PDF&petro&E&mean&yes&NoWF&0.3552&0.5266&0.6734&0.7338\\
PDF&petro&G&mean&yes&NoWF&0.3545&0.5287&0.6733&0.7322\\
\cline{1-10}
PDF&psf&O2&gmedian&yes&NoWF&0.4081&0.6106&0.7621&0.8152\\
PDF&psf&A&gmedian&yes&NoWF&0.4144&0.6142&0.7619&0.8115\\
PDF&psf&C&gmedian&yes&NoWF&0.4078&0.6046&0.7471&0.7939\\
PDF&psf&E&gmedian&yes&NoWF&0.4170&0.6042&0.7459&0.7937\\
PDF&psf&G&gmedian&yes&NoWF&0.4228&0.6082&0.7447&0.7933\\
PDF&model&O2&gmedian&yes&NoWF&0.4148&0.6147&0.7617&0.8134\\
PDF&model&A&gmedian&yes&NoWF&0.4278&0.6240&0.7704&0.8186\\
PDF&model&C&gmedian&yes&NoWF&0.4234&0.6169&0.7585&0.8043\\
PDF&model&E&gmedian&yes&NoWF&0.4377&0.6201&0.7562&0.8055\\
PDF&model&G&gmedian&yes&NoWF&0.4395&0.6194&0.7531&0.8026\\
PDF&fiber&O2&gmedian&yes&NoWF&0.4020&0.6019&0.7567&0.8083\\
PDF&fiber&A&gmedian&yes&NoWF&0.3996&0.5914&0.7400&0.7899\\
PDF&fiber&C&gmedian&yes&NoWF&0.4003&0.5901&0.7373&0.7853\\
PDF&fiber&E&gmedian&yes&NoWF&0.4117&0.5950&0.7309&0.7803\\
PDF&fiber&G&gmedian&yes&NoWF&0.4150&0.5953&0.7319&0.7809\\
PDF&petro&O2&gmedian&yes&NoWF&0.3386&0.5237&0.6918&0.7548\\
PDF&petro&A&gmedian&yes&NoWF&0.3551&0.5385&0.7001&0.7575\\
PDF&petro&C&gmedian&yes&NoWF&0.3432&0.5202&0.6756&0.7305\\
PDF&petro&E&gmedian&yes&NoWF&0.3519&0.5220&0.6665&0.7270\\
PDF&petro&G&gmedian&yes&NoWF&0.3499&0.5203&0.6623&0.7208\\
\cline{1-10}
PDF&psf&O2&gmode&yes&NoWF&0.3964&0.5947&0.7482&0.8037\\
PDF&psf&A&gmode&yes&NoWF&0.3955&0.5928&0.7397&0.7890\\
PDF&psf&C&gmode&yes&NoWF&0.3918&0.5861&0.7281&0.7746\\
PDF&psf&E&gmode&yes&NoWF&0.3971&0.5838&0.7252&0.7727\\
PDF&psf&G&gmode&yes&NoWF&0.3998&0.5830&0.7238&0.7745\\
PDF&model&O2&gmode&yes&NoWF&0.3954&0.5970&0.7443&0.7968\\
PDF&model&A&gmode&yes&NoWF&0.4062&0.5985&0.7452&0.7930\\
PDF&model&C&gmode&yes&NoWF&0.4059&0.5979&0.7415&0.7880\\
PDF&model&E&gmode&yes&NoWF&0.4152&0.6029&0.7420&0.7927\\
PDF&model&G&gmode&yes&NoWF&0.4064&0.5883&0.7316&0.7834\\
PDF&fiber&O2&gmode&yes&NoWF&0.3895&0.5884&0.7435&0.7963\\
PDF&fiber&A&gmode&yes&NoWF&0.3856&0.5820&0.7337&0.7871\\
PDF&fiber&C&gmode&yes&NoWF&0.3736&0.5629&0.7110&0.7619\\
PDF&fiber&E&gmode&yes&NoWF&0.3820&0.5662&0.7104&0.7621\\
PDF&fiber&G&gmode&yes&NoWF&0.3827&0.5685&0.7102&0.7639\\
PDF&petro&O2&gmode&yes&NoWF&0.3169&0.4941&0.6518&0.7191\\
PDF&petro&A&gmode&yes&NoWF&0.3376&0.5209&0.6811&0.7461\\
PDF&petro&C&gmode&yes&NoWF&0.3299&0.5073&0.6613&0.7234\\
PDF&petro&E&gmode&yes&NoWF&0.3315&0.5010&0.6505&0.7131\\
PDF&petro&G&gmode&yes&NoWF&0.3255&0.5008&0.6537&0.7156
     \enddata
     \end{deluxetable}
       
     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for high-redshift quasars using No Weighting Function and removing reddened quasars.  \label{PDFnoWFremovered_hightable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3303&0.5189&0.7458&0.8403\\
\cline{1-10}
PDF&psf&O2&mean&yes&NoWF&0.2762&0.4692&0.6767&0.7601\\
PDF&psf&A&mean&yes&NoWF&0.2484&0.4427&0.6476&0.7211\\
PDF&psf&C&mean&yes&NoWF&0.2559&0.4862&0.7217&0.8364\\
PDF&psf&E&mean&yes&NoWF&0.2565&0.4808&0.7124&0.8292\\
PDF&psf&G&mean&yes&NoWF&0.2557&0.4731&0.7037&0.8198\\
PDF&model&O2&mean&yes&NoWF&0.2841&0.4729&0.6796&0.7609\\
PDF&model&A&mean&yes&NoWF&0.2544&0.4510&0.6529&0.7250\\
PDF&model&C&mean&yes&NoWF&0.2573&0.4902&0.7222&0.8369\\
PDF&model&E&mean&yes&NoWF&0.2576&0.4833&0.7145&0.8307\\
PDF&model&G&mean&yes&NoWF&0.2591&0.4765&0.7068&0.8240\\
PDF&fiber&O2&mean&yes&NoWF&0.2484&0.4348&0.6604&0.7440\\
PDF&fiber&A&mean&yes&NoWF&0.2272&0.4129&0.6156&0.6903\\
PDF&fiber&C&mean&yes&NoWF&0.2600&0.4930&0.7208&0.8308\\
PDF&fiber&E&mean&yes&NoWF&0.2603&0.4958&0.7261&0.8415\\
PDF&fiber&G&mean&yes&NoWF&0.2577&0.4828&0.7190&0.8380\\
PDF&petro&O2&mean&yes&NoWF&0.1965&0.3508&0.5662&0.6591\\
PDF&petro&A&mean&yes&NoWF&0.1836&0.3395&0.5261&0.6156\\
PDF&petro&C&mean&yes&NoWF&0.2226&0.4290&0.6585&0.7797\\
PDF&petro&E&mean&yes&NoWF&0.2200&0.4270&0.6580&0.7831\\
PDF&petro&G&mean&yes&NoWF&0.2208&0.4218&0.6552&0.7825\\
\cline{1-10}
PDF&psf&O2&gmedian&yes&NoWF&0.2710&0.4623&0.6687&0.7536\\
PDF&psf&A&gmedian&yes&NoWF&0.2535&0.4506&0.6585&0.7289\\
PDF&psf&C&gmedian&yes&NoWF&0.2532&0.4848&0.7210&0.8357\\
PDF&psf&E&gmedian&yes&NoWF&0.2552&0.4773&0.7107&0.8280\\
PDF&psf&G&gmedian&yes&NoWF&0.2513&0.4724&0.7070&0.8262\\
PDF&model&O2&gmedian&yes&NoWF&0.2831&0.4690&0.6699&0.7542\\
PDF&model&A&gmedian&yes&NoWF&0.2594&0.4582&0.6623&0.7341\\
PDF&model&C&gmedian&yes&NoWF&0.2541&0.4845&0.7209&0.8361\\
PDF&model&E&gmedian&yes&NoWF&0.2563&0.4789&0.7152&0.8320\\
PDF&model&G&gmedian&yes&NoWF&0.2561&0.4737&0.7103&0.8285\\
PDF&fiber&O2&gmedian&yes&NoWF&0.2525&0.4376&0.6606&0.7432\\
PDF&fiber&A&gmedian&yes&NoWF&0.2310&0.4170&0.6210&0.6940\\
PDF&fiber&C&gmedian&yes&NoWF&0.2601&0.4937&0.7203&0.8298\\
PDF&fiber&E&gmedian&yes&NoWF&0.2575&0.4938&0.7225&0.8387\\
PDF&fiber&G&gmedian&yes&NoWF&0.2569&0.4832&0.7192&0.8413\\
PDF&petro&O2&gmedian&yes&NoWF&0.1936&0.3493&0.5667&0.6552\\
PDF&petro&A&gmedian&yes&NoWF&0.1874&0.3448&0.5287&0.6158\\
PDF&petro&C&gmedian&yes&NoWF&0.2236&0.4278&0.6590&0.7807\\
PDF&petro&E&gmedian&yes&NoWF&0.2213&0.4283&0.6603&0.7856\\
PDF&petro&G&gmedian&yes&NoWF&0.2216&0.4234&0.6582&0.7856\\
\cline{1-10}
PDF&psf&O2&gmode&yes&NoWF&0.2775&0.4615&0.6759&0.7762\\
PDF&psf&A&gmode&yes&NoWF&0.2594&0.4628&0.6845&0.7648\\
PDF&psf&C&gmode&yes&NoWF&0.2437&0.4724&0.7212&0.8527\\
PDF&psf&E&gmode&yes&NoWF&0.2473&0.4688&0.7129&0.8408\\
PDF&psf&G&gmode&yes&NoWF&0.2382&0.4568&0.7073&0.8390\\
PDF&model&O2&gmode&yes&NoWF&0.2874&0.4710&0.6821&0.7759\\
PDF&model&A&gmode&yes&NoWF&0.2698&0.4715&0.6874&0.7638\\
PDF&model&C&gmode&yes&NoWF&0.2459&0.4774&0.7252&0.8551\\
PDF&model&E&gmode&yes&NoWF&0.2535&0.4811&0.7288&0.8550\\
PDF&model&G&gmode&yes&NoWF&0.2446&0.4651&0.7129&0.8425\\
PDF&fiber&O2&gmode&yes&NoWF&0.2561&0.4306&0.6600&0.7543\\
PDF&fiber&A&gmode&yes&NoWF&0.2426&0.4347&0.6487&0.7303\\
PDF&fiber&C&gmode&yes&NoWF&0.2578&0.4917&0.7277&0.8421\\
PDF&fiber&E&gmode&yes&NoWF&0.2521&0.4873&0.7253&0.8400\\
PDF&fiber&G&gmode&yes&NoWF&0.2500&0.4740&0.7177&0.8375\\
PDF&petro&O2&gmode&yes&NoWF&0.2016&0.3552&0.5767&0.6756\\
PDF&petro&A&gmode&yes&NoWF&0.2112&0.3837&0.5734&0.6581\\
PDF&petro&C&gmode&yes&NoWF&0.2244&0.4300&0.6670&0.7999\\
PDF&petro&E&gmode&yes&NoWF&0.2200&0.4303&0.6700&0.8043\\
PDF&petro&G&gmode&yes&NoWF&0.2195&0.4173&0.6521&0.7762
     \enddata
     \end{deluxetable}       
     
     \clearpage
     
     \begin{deluxetable}{c c c c c c || c c c c | c c | c c | c c | c }
     \rotate
     \tablecolumns{17}
     \tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{All} & \multicolumn{7}{c}{Catastrophic Failures} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$} & 
     \colhead{\# CF} & 
     \colhead{\% CF} & 
     \colhead{\# Common} & 
     \colhead{\%} &
     \colhead{\# Diff} & 
     \colhead{\%} & 
     \colhead{\# not CF}}
     \tablecaption{PDF Photometric Redshift Estimates using No Weighting Function, without removing reddened quasars.  \label{PDFnoWFnoremovered_table}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3835&0.5889&0.7648&0.8232&6821&0.1469&NA&NA&NA&NA&NA\\
\cline{1-17}
PDF&psf&O2&mean&no&NoWF&0.3751&0.5784&0.7526&0.8091&7442&0.1603&4137&0.5559&2822&0.3792&2684\\
PDF&psf&A&mean&no&NoWF&0.3690&0.5703&0.7455&0.7999&7837&0.1688&4025&0.5136&3296&0.4206&2796\\
PDF&psf&C&mean&no&NoWF&0.3708&0.5753&0.7492&0.8044&7630&0.1644&4166&0.5460&2958&0.3877&2655\\
PDF&psf&E&mean&no&NoWF&0.3811&0.5813&0.7500&0.8045&7554&0.1627&4122&0.5457&2927&0.3875&2699\\
PDF&psf&G&mean&no&NoWF&0.3888&0.5891&0.7482&0.8045&7544&0.1625&4192&0.5557&2835&0.3758&2629\\
PDF&model&O2&mean&no&NoWF&0.3794&0.5792&0.7472&0.8027&7796&0.1682&4024&0.5162&3252&0.4171&2797\\
PDF&model&A&mean&no&NoWF&0.3710&0.5704&0.7446&0.7976&7966&0.1718&4004&0.5026&3431&0.4307&2817\\
PDF&model&C&mean&no&NoWF&0.3775&0.5801&0.7545&0.8088&7427&0.1602&4073&0.5484&2859&0.3849&2748\\
PDF&model&E&mean&no&NoWF&0.3900&0.5892&0.7564&0.8112&7272&0.1569&4022&0.5531&2769&0.3808&2799\\
PDF&model&G&mean&no&NoWF&0.4021&0.6026&0.7583&0.8149&7087&0.1529&4103&0.5789&2510&0.3542&2718\\
PDF&fiber&O2&mean&no&NoWF&0.3667&0.5630&0.7369&0.7937&8060&0.1739&3955&0.4907&3566&0.4424&2866\\
PDF&fiber&A&mean&no&NoWF&0.3543&0.5481&0.7188&0.7719&9073&0.1957&3986&0.4393&4465&0.4921&2835\\
PDF&fiber&C&mean&no&NoWF&0.3667&0.5660&0.7398&0.7947&8017&0.1729&4028&0.5024&3455&0.4310&2793\\
PDF&fiber&E&mean&no&NoWF&0.3805&0.5760&0.7390&0.7952&7906&0.1705&4000&0.5059&3388&0.4285&2821\\
PDF&fiber&G&mean&no&NoWF&0.3862&0.5814&0.7388&0.7966&7803&0.1683&4013&0.5143&3274&0.4196&2808\\
PDF&petro&O2&mean&no&NoWF&0.2864&0.4620&0.6419&0.7137&10803&0.2330&3844&0.3558&6258&0.5793&2977\\
PDF&petro&A&mean&no&NoWF&0.2940&0.4727&0.6485&0.7140&11087&0.2392&3744&0.3377&6648&0.5996&3077\\
PDF&petro&C&mean&no&NoWF&0.3014&0.4838&0.6607&0.7257&10505&0.2266&3742&0.3562&6112&0.5818&3079\\
PDF&petro&E&mean&no&NoWF&0.3115&0.4877&0.6587&0.7241&10494&0.2264&3713&0.3538&6134&0.5845&3108\\
PDF&petro&G&mean&no&NoWF&0.3206&0.5004&0.6631&0.7313&10098&0.2178&3834&0.3797&5628&0.5573&2987\\
\cline{1-17}
PDF&psf&O2&gmedian&no&NoWF&0.3749&0.5776&0.7519&0.8098&7403&0.1595&4177&0.5642&2741&0.3703&2644\\
PDF&psf&A&gmedian&no&NoWF&0.3659&0.5663&0.7439&0.8000&7774&0.1675&4042&0.5199&3205&0.4123&2779\\
PDF&psf&C&gmedian&no&NoWF&0.3684&0.5714&0.7466&0.8037&7585&0.1634&4175&0.5504&2901&0.3825&2646\\
PDF&psf&E&gmedian&no&NoWF&0.3805&0.5810&0.7497&0.8057&7512&0.1618&4174&0.5556&3338&0.4444&2647\\
PDF&psf&G&gmedian&no&NoWF&0.3865&0.5855&0.7474&0.8067&7402&0.1595&4234&0.5720&2683&0.3625&2587\\
PDF&model&O2&gmedian&no&NoWF&0.3741&0.5732&0.7415&0.7990&7924&0.1709&4113&0.5191&3280&0.4139&2708\\
PDF&model&A&gmedian&no&NoWF&0.3689&0.5681&0.7435&0.7988&7838&0.1691&4009&0.5115&3312&0.4226&2812\\
PDF&model&C&gmedian&no&NoWF&0.3724&0.5725&0.7469&0.8032&7606&0.1641&4126&0.5425&2975&0.3911&2695\\
PDF&model&E&gmedian&no&NoWF&0.3900&0.5870&0.7542&0.8111&7283&0.1571&4068&0.5586&2735&0.3755&2753\\
PDF&model&G&gmedian&no&NoWF&0.4007&0.5972&0.7536&0.8134&7105&0.1533&4167&0.5865&2465&0.3469&2654\\
PDF&fiber&O2&gmedian&no&NoWF&0.3665&0.5635&0.7385&0.7969&7913&0.1707&3998&0.5052&3375&0.4265&2823\\
PDF&fiber&A&gmedian&no&NoWF&0.3538&0.5473&0.7183&0.7736&8926&0.1925&4033&0.4518&4282&0.4797&2788\\
PDF&fiber&C&gmedian&no&NoWF&0.3641&0.5629&0.7361&0.7931&8016&0.1729&4064&0.5070&3408&0.4251&2757\\
PDF&fiber&E&gmedian&no&NoWF&0.3803&0.5733&0.7374&0.7959&7829&0.1689&4038&0.5158&3275&0.4183&2783\\
PDF&fiber&G&gmedian&no&NoWF&0.3826&0.5774&0.7356&0.7962&7738&0.1669&4048&0.5231&3167&0.4093&2773\\
PDF&petro&O2&gmedian&no&NoWF&0.2837&0.4574&0.6336&0.7053&11163&0.2408&3931&0.3521&6519&0.5840&2890\\
PDF&petro&A&gmedian&no&NoWF&0.2930&0.4727&0.6481&0.7159&10864&0.2344&3749&0.3451&6431&0.5920&3072\\
PDF&petro&C&gmedian&no&NoWF&0.2950&0.4765&0.6514&0.7179&10727&0.2314&3791&0.3534&6262&0.5838&3030\\
PDF&petro&E&gmedian&no&NoWF&0.3088&0.4831&0.6531&0.7203&10583&0.2283&3778&0.3570&6136&0.5798&3043\\
PDF&petro&G&gmedian&no&NoWF&0.3187&0.4970&0.6605&0.7297&10125&0.2184&3906&0.3858&5569&0.5500&2915\\
\cline{1-17}
PDF&psf&O2&gmode&no&NoWF&0.3638&0.5638&0.7392&0.8046&7487&0.1613&4204&0.5615&2795&0.3733&2617\\
PDF&psf&A&gmode&no&NoWF&0.3598&0.5616&0.7380&0.7978&7688&0.1656&4179&0.5436&2989&0.3888&2642\\
PDF&psf&C&gmode&no&NoWF&0.3615&0.5658&0.7403&0.8019&7485&0.1612&4367&0.5834&2611&0.3488&2454\\
PDF&psf&E&gmode&no&NoWF&0.3715&0.5717&0.7412&0.8010&7597&0.1637&4376&0.5760&3221&0.4240&2445\\
PDF&psf&G&gmode&no&NoWF&0.3755&0.5728&0.7381&0.8040&7330&0.1579&4364&0.5954&2966&0.4046&2457\\
PDF&model&O2&gmode&no&NoWF&0.3597&0.5602&0.7290&0.7950&8002&0.1726&4281&0.5350&3187&0.3983&2540\\
PDF&model&A&gmode&no&NoWF&0.3557&0.5539&0.7336&0.7893&8203&0.1769&4228&0.5154&3410&0.4157&2593\\
PDF&model&C&gmode&no&NoWF&0.3634&0.5642&0.7428&0.8004&7612&0.1642&4274&0.5615&2834&0.3723&2547\\
PDF&model&E&gmode&no&NoWF&0.3765&0.5760&0.7478&0.8058&7407&0.1598&4269&0.5763&2640&0.3564&2552\\
PDF&model&G&gmode&no&NoWF&0.3756&0.5704&0.7351&0.8046&7255&0.1565&4244&0.5850&2521&0.3475&2577\\
PDF&fiber&O2&gmode&no&NoWF&0.3565&0.5526&0.7307&0.7957&7743&0.1670&4067&0.5252&3139&0.4054&2754\\
PDF&fiber&A&gmode&no&NoWF&0.3463&0.5475&0.7227&0.7821&8372&0.1806&4101&0.4898&3711&0.4433&2720\\
PDF&fiber&C&gmode&no&NoWF&0.3469&0.5480&0.7205&0.7806&8452&0.1823&4266&0.5047&3610&0.4271&2555\\
PDF&fiber&E&gmode&no&NoWF&0.3622&0.5570&0.7221&0.7836&8315&0.1794&4258&0.5121&3495&0.4203&2563\\
PDF&fiber&G&gmode&no&NoWF&0.3617&0.5551&0.7162&0.7791&8425&0.1817&4222&0.5011&3625&0.4303&2599\\
PDF&petro&O2&gmode&no&NoWF&0.2655&0.4366&0.6122&0.6874&11652&0.2514&3991&0.3425&6881&0.5905&2830\\
PDF&petro&A&gmode&no&NoWF&0.2850&0.4647&0.6384&0.7131&10835&0.2337&3792&0.3500&6362&0.5872&3029\\
PDF&petro&C&gmode&no&NoWF&0.2876&0.4686&0.6421&0.7165&10682&0.2304&3837&0.3592&6164&0.5770&2984\\
PDF&petro&E&gmode&no&NoWF&0.2966&0.4700&0.6407&0.7145&10571&0.2280&3827&0.3620&6063&0.5736&2994\\
PDF&petro&G&gmode&no&NoWF&0.2983&0.4799&0.6536&0.7247&10174&0.2195&4026&0.3957&5513&0.5419&2795
     \enddata
     \end{deluxetable}     
     
     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for low-redshift quasars using No Weighting Function without removing reddened quasars.  \label{PDFnoWFnoremovered_lowtable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3947&0.6036&0.7689&0.8196\\
\cline{1-10}
PDF&psf&O2&mean&no&NoWF&0.4099&0.6230&0.7927&0.8454\\
PDF&psf&A&mean&no&NoWF&0.4057&0.6164&0.7892&0.8408\\
PDF&psf&C&mean&no&NoWF&0.3920&0.5962&0.7655&0.8146\\
PDF&psf&E&mean&no&NoWF&0.4044&0.6037&0.7668&0.8148\\
PDF&psf&G&mean&no&NoWF&0.4138&0.6128&0.7638&0.8140\\
PDF&model&O2&mean&no&NoWF&0.4124&0.6206&0.7832&0.8348\\
PDF&model&A&mean&no&NoWF&0.4073&0.6146&0.7867&0.8368\\
PDF&model&C&mean&no&NoWF&0.3994&0.6018&0.7711&0.8192\\
PDF&model&E&mean&no&NoWF&0.4142&0.6123&0.7736&0.8218\\
PDF&model&G&mean&no&NoWF&0.4289&0.6281&0.7748&0.8252\\
PDF&fiber&O2&mean&no&NoWF&0.3998&0.6042&0.7751&0.8288\\
PDF&fiber&A&mean&no&NoWF&0.3886&0.5903&0.7598&0.8101\\
PDF&fiber&C&mean&no&NoWF&0.3863&0.5851&0.7546&0.8038\\
PDF&fiber&E&mean&no&NoWF&0.4027&0.5968&0.7537&0.8041\\
PDF&fiber&G&mean&no&NoWF&0.4096&0.6028&0.7518&0.8032\\
PDF&petro&O2&mean&no&NoWF&0.3163&0.5033&0.6857&0.7548\\
PDF&petro&A&mean&no&NoWF&0.3263&0.5175&0.6976&0.7597\\
PDF&petro&C&mean&no&NoWF&0.3179&0.5031&0.6779&0.7380\\
PDF&petro&E&mean&no&NoWF&0.3305&0.5088&0.6763&0.7365\\
PDF&petro&G&mean&no&NoWF&0.3419&0.5235&0.6801&0.7427\\
\cline{1-10}
PDF&psf&O2&gmedian&no&NoWF&0.4089&0.6192&0.7888&0.8434\\
PDF&psf&A&gmedian&no&NoWF&0.4010&0.6094&0.7840&0.8382\\
PDF&psf&C&gmedian&no&NoWF&0.3886&0.5905&0.7611&0.8128\\
PDF&psf&E&gmedian&no&NoWF&0.4029&0.6015&0.7643&0.8142\\
PDF&psf&G&gmedian&no&NoWF&0.4105&0.6065&0.7596&0.8123\\
PDF&model&O2&gmedian&no&NoWF&0.4047&0.6112&0.7742&0.8284\\
PDF&model&A&gmedian&no&NoWF&0.4038&0.6097&0.7822&0.8352\\
PDF&model&C&gmedian&no&NoWF&0.3932&0.5926&0.7614&0.8118\\
PDF&model&E&gmedian&no&NoWF&0.4138&0.6086&0.7689&0.8192\\
PDF&model&G&gmedian&no&NoWF&0.4270&0.6208&0.7667&0.8197\\
PDF&fiber&O2&gmedian&no&NoWF&0.3979&0.6015&0.7745&0.8304\\
PDF&fiber&A&gmedian&no&NoWF&0.3862&0.5869&0.7560&0.8095\\
PDF&fiber&C&gmedian&no&NoWF&0.3827&0.5802&0.7487&0.8008\\
PDF&fiber&E&gmedian&no&NoWF&0.4017&0.5918&0.7495&0.8029\\
PDF&fiber&G&gmedian&no&NoWF&0.4048&0.5956&0.7447&0.7985\\
PDF&petro&O2&gmedian&no&NoWF&0.3111&0.4952&0.6739&0.7445\\
PDF&petro&A&gmedian&no&NoWF&0.3239&0.5158&0.6953&0.7610\\
PDF&petro&C&gmedian&no&NoWF&0.3107&0.4942&0.6668&0.7294\\
PDF&petro&E&gmedian&no&NoWF&0.3268&0.5016&0.6678&0.7305\\
PDF&petro&G&gmedian&no&NoWF&0.3388&0.5168&0.6735&0.7368\\
\cline{1-10}
PDF&psf&O2&gmode&no&NoWF&0.3961&0.6045&0.7750&0.8337\\
PDF&psf&A&gmode&no&NoWF&0.3913&0.6013&0.7722&0.8296\\
PDF&psf&C&gmode&no&NoWF&0.3814&0.5848&0.7519&0.8064\\
PDF&psf&E&gmode&no&NoWF&0.3938&0.5923&0.7539&0.8060\\
PDF&psf&G&gmode&no&NoWF&0.4002&0.5952&0.7495&0.8065\\
PDF&model&O2&gmode&no&NoWF&0.3853&0.5929&0.7548&0.8167\\
PDF&model&A&gmode&no&NoWF&0.3842&0.5872&0.7626&0.8152\\
PDF&model&C&gmode&no&NoWF&0.3826&0.5814&0.7538&0.8043\\
PDF&model&E&gmode&no&NoWF&0.3980&0.5947&0.7592&0.8092\\
PDF&model&G&gmode&no&NoWF&0.3990&0.5908&0.7446&0.8062\\
PDF&fiber&O2&gmode&no&NoWF&0.3856&0.5887&0.7609&0.8215\\
PDF&fiber&A&gmode&no&NoWF&0.3760&0.5839&0.7548&0.8124\\
PDF&fiber&C&gmode&no&NoWF&0.3618&0.5614&0.7281&0.7825\\
PDF&fiber&E&gmode&no&NoWF&0.3802&0.5720&0.7301&0.7857\\
PDF&fiber&G&gmode&no&NoWF&0.3819&0.5728&0.7240&0.7805\\
PDF&petro&O2&gmode&no&NoWF&0.2876&0.4679&0.6444&0.7170\\
PDF&petro&A&gmode&no&NoWF&0.3123&0.5016&0.6783&0.7523\\
PDF&petro&C&gmode&no&NoWF&0.3014&0.4830&0.6523&0.7229\\
PDF&petro&E&gmode&no&NoWF&0.3132&0.4864&0.6507&0.7194\\
PDF&petro&G&gmode&no&NoWF&0.3162&0.4985&0.6662&0.7315
     \enddata
     \end{deluxetable}
     
     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for high-redshift quasars using No Weighting Function without removing reddened quasars.  \label{PDFnoWFnoremovered_hightable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3303&0.5189&0.7458&0.8403\\
\cline{1-10}
PDF&psf&O2&mean&no&NoWF&0.2096&0.3662&0.5616&0.6366\\
PDF&psf&A&mean&no&NoWF&0.1943&0.3516&0.5380&0.6056\\
PDF&psf&C&mean&no&NoWF&0.2305&0.4372&0.6418&0.7371\\
PDF&psf&E&mean&no&NoWF&0.2267&0.4334&0.6390&0.7364\\
PDF&psf&G&mean&no&NoWF&0.2239&0.4328&0.6454&0.7419\\
PDF&model&O2&mean&no&NoWF&0.2225&0.3821&0.5761&0.6498\\
PDF&model&A&mean&no&NoWF&0.1984&0.3604&0.5444&0.6113\\
PDF&model&C&mean&no&NoWF&0.2325&0.4369&0.6451&0.7403\\
PDF&model&E&mean&no&NoWF&0.2307&0.4361&0.6427&0.7414\\
PDF&model&G&mean&no&NoWF&0.2253&0.4341&0.6492&0.7470\\
PDF&fiber&O2&mean&no&NoWF&0.2094&0.3672&0.5554&0.6266\\
PDF&fiber&A&mean&no&NoWF&0.1915&0.3476&0.5240&0.5902\\
PDF&fiber&C&mean&no&NoWF&0.2368&0.4397&0.6425&0.7349\\
PDF&fiber&E&mean&no&NoWF&0.2342&0.4389&0.6424&0.7364\\
PDF&fiber&G&mean&no&NoWF&0.2312&0.4405&0.6526&0.7527\\
PDF&petro&O2&mean&no&NoWF&0.1442&0.2657&0.4336&0.5185\\
PDF&petro&A&mean&no&NoWF&0.1403&0.2601&0.4152&0.4968\\
PDF&petro&C&mean&no&NoWF&0.1919&0.3561&0.5470&0.6444\\
PDF&petro&E&mean&no&NoWF&0.1858&0.3477&0.5421&0.6419\\
PDF&petro&G&mean&no&NoWF&0.1799&0.3476&0.5505&0.6554\\
\cline{1-10}
PDF&psf&O2&gmedian&no&NoWF&0.2136&0.3799&0.5768&0.6500\\
PDF&psf&A&gmedian&no&NoWF&0.1991&0.3615&0.5538&0.6185\\
PDF&psf&C&gmedian&no&NoWF&0.2354&0.4450&0.6513&0.7438\\
PDF&psf&E&gmedian&no&NoWF&0.2321&0.4457&0.6536&0.7492\\
PDF&psf&G&gmedian&no&NoWF&0.2282&0.4464&0.6665&0.7692\\
PDF&model&O2&gmedian&no&NoWF&0.2286&0.3929&0.5861&0.6592\\
PDF&model&A&gmedian&no&NoWF&0.2030&0.3702&0.5597&0.6258\\
PDF&model&C&gmedian&no&NoWF&0.2348&0.4397&0.6509&0.7463\\
PDF&model&E&gmedian&no&NoWF&0.2328&0.4440&0.6571&0.7573\\
PDF&model&G&gmedian&no&NoWF&0.2269&0.4412&0.6671&0.7719\\
PDF&fiber&O2&gmedian&no&NoWF&0.2169&0.3826&0.5677&0.6377\\
PDF&fiber&A&gmedian&no&NoWF&0.1997&0.3589&0.5391&0.6029\\
PDF&fiber&C&gmedian&no&NoWF&0.2408&0.4485&0.6527&0.7425\\
PDF&fiber&E&gmedian&no&NoWF&0.2386&0.4510&0.6570&0.7500\\
PDF&fiber&G&gmedian&no&NoWF&0.2355&0.4566&0.6759&0.7807\\
PDF&petro&O2&gmedian&no&NoWF&0.1535&0.2780&0.4420&0.5191\\
PDF&petro&A&gmedian&no&NoWF&0.1459&0.2679&0.4235&0.5014\\
PDF&petro&C&gmedian&no&NoWF&0.1911&0.3600&0.5495&0.6419\\
PDF&petro&E&gmedian&no&NoWF&0.1904&0.3609&0.5561&0.6528\\
PDF&petro&G&gmedian&no&NoWF&0.1863&0.3663&0.5748&0.6835\\
\cline{1-10}
PDF&psf&O2&gmode&no&NoWF&0.2104&0.3702&0.5692&0.6660\\
PDF&psf&A&gmode&no&NoWF&0.2101&0.3731&0.5756&0.6468\\
PDF&psf&C&gmode&no&NoWF&0.2305&0.4410&0.6640&0.7720\\
PDF&psf&E&gmode&no&NoWF&0.2244&0.4354&0.6578&0.7677\\
PDF&psf&G&gmode&no&NoWF&0.2126&0.4254&0.6624&0.7876\\
PDF&model&O2&gmode&no&NoWF&0.2379&0.4048&0.6064&0.6916\\
PDF&model&A&gmode&no&NoWF&0.2207&0.3955&0.5953&0.6662\\
PDF&model&C&gmode&no&NoWF&0.2364&0.4505&0.6701&0.7741\\
PDF&model&E&gmode&no&NoWF&0.2345&0.4528&0.6724&0.7834\\
PDF&model&G&gmode&no&NoWF&0.2207&0.4358&0.6722&0.7941\\
PDF&fiber&O2&gmode&no&NoWF&0.2179&0.3810&0.5871&0.6733\\
PDF&fiber&A&gmode&no&NoWF&0.2051&0.3745&0.5701&0.6383\\
PDF&fiber&C&gmode&no&NoWF&0.2486&0.4594&0.6701&0.7676\\
PDF&fiber&E&gmode&no&NoWF&0.2432&0.4577&0.6693&0.7699\\
PDF&fiber&G&gmode&no&NoWF&0.2283&0.4377&0.6650&0.7694\\
PDF&petro&O2&gmode&no&NoWF&0.1605&0.2879&0.4592&0.5468\\
PDF&petro&A&gmode&no&NoWF&0.1552&0.2892&0.4486&0.5268\\
PDF&petro&C&gmode&no&NoWF&0.1967&0.3738&0.5751&0.6741\\
PDF&petro&E&gmode&no&NoWF&0.1867&0.3620&0.5748&0.6820\\
PDF&petro&G&gmode&no&NoWF&0.1801&0.3574&0.5700&0.6795
     \enddata
     \end{deluxetable}

\clearpage

     \begin{deluxetable}{c c c c c c || c c c c | c c | c c | c c | c }
     \rotate
     \tablecolumns{17}
     \tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{All} & \multicolumn{7}{c}{Catastrophic Failures} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$} & 
     \colhead{\# CF} & 
     \colhead{\% CF} & 
     \colhead{\# Common} & 
     \colhead{\%} &
     \colhead{\# Diff} & 
     \colhead{\%} & 
     \colhead{\# not CF}}
     \tablecaption{PDF Photometric Redshift Estimates using combinations of PDFs from different magnitudes without removing reddened quasars.  \label{PDFmultimagsO2}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3835&0.5889&0.7648&0.8232&6821&0.1469&NA&NA&NA&NA&NA\\
\cline{1-17}
PDF&psfmodel&O2&mean&no&SimpleWF&0.3691&0.5775&0.7693&0.8273&6699&0.1445&4832&0.7213&1411&0.2106&1989\\
PDF&psffiber&O2&mean&no&SimpleWF&0.3688&0.5769&0.7697&0.8272&6744&0.1455&4780&0.7088&1495&0.2217&2041\\
PDF&psfpetro&O2&mean&no&SimpleWF&0.3444&0.5469&0.7495&0.8148&7094&0.1530&4646&0.6549&1972&0.2780&2175\\
PDF&modelfiber&O2&mean&no&SimpleWF&0.3689&0.5755&0.7693&0.8273&6759&0.1458&4694&0.6945&1603&0.2372&2127\\
PDF&modelpetro&O2&mean&no&SimpleWF&0.3425&0.5437&0.7457&0.8114&7255&0.1565&4616&0.6363&2176&0.2999&2205\\
PDF&fiberpetro&O2&mean&no&SimpleWF&0.3303&0.5278&0.7303&0.7994&7619&0.1644&4511&0.5921&2596&0.3407&2310\\
\cline{1-17}
PDF&psfmodelfiber&O2&mean&no&SimpleWF&0.3707&0.5789&0.7712&0.8286&6689&0.1443&4790&0.7161&1439&0.2151&2031\\
PDF&psfmodelpetro&O2&mean&no&SimpleWF&0.3579&0.5615&0.7594&0.8215&6919&0.1493&4691&0.6780&1763&0.2548&2130\\
PDF&psffiberpetro&O2&mean&no&SimpleWF&0.3539&0.5564&0.7564&0.8193&6968&0.1503&4634&0.6650&1866&0.2678&2187\\
PDF&modelfiberpetro&O2&mean&no&SimpleWF&0.3530&0.5540&0.7537&0.8176&7068&0.1525&4602&0.6511&2001&0.2831&2219\\
\cline{1-17}
PDF&allmags&O2&mean&no&SimpleWF&0.3612&0.5644&0.7621&0.8236&6855&0.1479&4679&0.6826&1714&0.2500&2142\\
PDF&allmags&O2&mean&no&NoWF&0.3752&0.5752&0.7507&0.8089&7448&0.1607&4021&0.5399&2944&0.3953&2800
     \enddata
     \end{deluxetable}
     
     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for low-redshift quasars using combinations of PDFs from different magnitudes without removing reddened quasars. \label{PDFmultimagsO2lowtable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3947&0.6036&0.7689&0.8196\\
\cline{1-10}
PDF&psfmodel&O2&mean&no&SimpleWF&0.3843&0.6006&0.7861&0.8387\\
PDF&psffiber&O2&mean&no&SimpleWF&0.3844&0.5988&0.7845&0.8362\\
PDF&psfpetro&O2&mean&no&SimpleWF&0.3580&0.5668&0.7646&0.8238\\
PDF&modelfiber&O2&mean&no&SimpleWF&0.3840&0.5968&0.7842&0.8365\\
PDF&modelpetro&O2&mean&no&SimpleWF&0.3559&0.5631&0.7607&0.8206\\
PDF&fiberpetro&O2&mean&no&SimpleWF&0.3427&0.5460&0.7434&0.8061\\
\cline{1-10}
PDF&psfmodelfiber&O2&mean&no&SimpleWF&0.3858&0.6003&0.7860&0.8378\\
PDF&psfmodelpetro&O2&mean&no&SimpleWF&0.3717&0.5819&0.7747&0.8308\\
PDF&psffiberpetro&O2&mean&no&SimpleWF&0.3675&0.5755&0.7698&0.8269\\
PDF&modelfiberpetro&O2&mean&no&SimpleWF&0.3665&0.5731&0.7675&0.8255\\
\cline{1-10}
PDF&allmags&O2&mean&no&SimpleWF&0.3756&0.5848&0.7768&0.8322\\
PDF&allmags&O2&mean&no&NoWF&0.4104&0.6189&0.7918&0.8465
     \enddata
     \end{deluxetable}
     
     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for high-redshift quasars using combinations of PDFs from different magnitudes without removing reddened quasars. \label{PDFmultimagsO2_hightable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3947&0.6036&0.7689&0.8196\\
\cline{1-10}
PDF&psfmodel&O2&mean&no&SimpleWF&0.2966&0.4681&0.6890&0.7729\\
PDF&psffiber&O2&mean&no&SimpleWF&0.2944&0.4727&0.6990&0.7844\\
PDF&psfpetro&O2&mean&no&SimpleWF&0.2797&0.4522&0.6777&0.7718\\
PDF&modelfiber&O2&mean&no&SimpleWF&0.2972&0.4738&0.6987&0.7831\\
PDF&modelpetro&O2&mean&no&SimpleWF&0.2790&0.4512&0.6744&0.7681\\
PDF&fiberpetro&O2&mean&no&SimpleWF&0.2715&0.4415&0.6677&0.7675\\
\cline{1-10}
PDF&psfmodelfiber&O2&mean&no&SimpleWF&0.2990&0.4774&0.7010&0.7850\\
PDF&psfmodelpetro&O2&mean&no&SimpleWF&0.2922&0.4649&0.6870&0.7774\\
PDF&psffiberpetro&O2&mean&no&SimpleWF&0.2890&0.4653&0.6924&0.7828\\
PDF&modelfiberpetro&O2&mean&no&SimpleWF&0.2890&0.4634&0.6879&0.7801\\
\cline{1-10}
PDF&allmags&O2&mean&no&SimpleWF&0.2926&0.4672&0.6923&0.7829\\
PDF&allmags&O2&mean&no&NoWF&0.2076&0.3672&0.5553&0.6303
     \enddata
     \end{deluxetable}     
     
          \begin{deluxetable}{c c c c c c || c c c c | c c | c c | c c | c }
     \rotate
     \tablecolumns{17}
     \tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{All} & \multicolumn{7}{c}{Catastrophic Failures} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$} & 
     \colhead{\# CF} & 
     \colhead{\% CF} & 
     \colhead{\# Common} & 
     \colhead{\%} &
     \colhead{\# Diff} & 
     \colhead{\%} & 
     \colhead{\# not CF}}
     \tablecaption{PDF Photometric Redshift Estimates using fewer colors.  \label{PDFfewercolorstable}}
     \startdata
PDF&psf UGRIZ&O2&mean&yes&SimpleWF&0.3835&0.5889&0.7648&0.8232&6821&0.1469&NA&NA&NA&NA&NA\\
PDF&psf UGRIZ&O2&mean&no&SimpleWF&0.3648&0.5736&0.7660&0.8242&6800&0.1465&4883&0.7181&1446&0.2126&1938\\
\cline{1-17}
PDF&psf UGR&O2&mean&no&SimpleWF&0.1724&0.3130&0.5034&0.5918&14775&0.3183&4948&0.3349&8729&0.5908&1873\\
PDF&psf GRI&O2&mean&no&SimpleWF&0.2050&0.3548&0.5282&0.6050&15241&0.3283&4909&0.3221&9261&0.6076&1912\\
PDF&psf RIZ&O2&mean&no&SimpleWF&0.2209&0.3768&0.5702&0.6586&13532&0.2915&4711&0.3481&7879&0.5822&2110\\
\cline{1-17}
PDF&psf UGRI&O2&mean&no&SimpleWF&0.2729&0.4577&0.6500&0.7195&10572&0.2278&4971&0.4702&4829&0.4568&1850\\
PDF&psf GRIZ&O2&mean&no&SimpleWF&0.3037&0.4844&0.6651&0.7271&10986&0.2367&4979&0.4532&5260&0.4788&1842\\
\cline{1-17}
\cline{1-17}
PDF&psf non-adj&O2&mean&no&SimpleWF&0.2573&0.4440&0.6438&0.7312&8585&0.1849&4680&0.5451&3904&0.4547&2142
\enddata
\end{deluxetable}


     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\rotate
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for low-redshift quasars using fewer colors.  \label{PDFfewercolors_lowtable}}
     \startdata
PDF&psf UGRIZ&O2&mean&yes&SimpleWF&0.3947&0.6036&0.7689&0.8196\\
PDF&psf UGRIZ&O2&mean&no&SimpleWF&0.3808&0.5970&0.7830&0.8359\\
\cline{1-10}
PDF&psf UGR&O2&mean&no&SimpleWF&0.1712&0.3114&0.4943&0.5745\\
PDF&psf GRI&O2&mean&no&SimpleWF&0.2171&0.3809&0.5650&0.6453\\
PDF&psf RIZ&O2&mean&no&SimpleWF&0.2343&0.4095&0.6236&0.7185\\
\cline{1-10}
PDF&psf UGRI&O2&mean&no&SimpleWF&0.2816&0.4719&0.6595&0.7248\\
PDF&psf GRIZ&O2&mean&no&SimpleWF&0.3283&0.5256&0.7128&0.7724\\
\cline{1-10}
\cline{1-10}
PDF&psf non-adj&O2&mean&no&SimpleWF&0.2528&0.4429&0.6395&0.7251
\enddata
\end{deluxetable}

     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\rotate
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for high-redshift quasars using fewer colors.  \label{PDFfewercolors_hightable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&0.3303&0.5189&0.7458&0.8403\\
PDF&psf&O2&mean&no&SimpleWF&0.2887&0.4624&0.6848&0.7687\\
\cline{1-10}
PDF&psf UGR&O2&mean&no&SimpleWF&0.1780&0.3209&0.5466&0.6739\\
PDF&psf GRI&O2&mean&no&SimpleWF&0.1479&0.2311&0.3534&0.4137\\
PDF&psf RIZ&O2&mean&no&SimpleWF&0.1575&0.2214&0.3164&0.3737\\
\cline{1-10}
PDF&psf UGRI&O2&mean&no&SimpleWF&0.2314&0.3902&0.6045&0.6947\\
PDF&psf GRIZ&O2&mean&no&SimpleWF&0.1870&0.2888&0.4386&0.5118\\
\cline{1-10}
\cline{1-10}
PDF&psf non-adj&O2&mean&no&SimpleWF&0.2788&0.4489&0.6645&0.7605
\enddata
\end{deluxetable}

     \begin{deluxetable}{c c c c c c || c c c c | c c }
     \tablecolumns{12}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{5}{c}{All} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$} & 
     \colhead{CF} & 
     \colhead{\% CF} }
     \tablecaption{Photometric Redshift Estimates: Comparison between using 4 colors and 5 colors for quasars with GALEX matches.  \label{sdssGalex_alltable}}
     \startdata
$\chi^2$&psf&O2&mean&no&N/A&0.4937&0.6880&0.8025&0.8402&2162&0.1415\\
PDF&psf&O2&mean&no&SimpleWF&0.5533&0.7429&0.8609&0.9004&1250&0.0818\\
$\chi^2$&psfgalex&O2&mean&no&N/A&0.5050&0.7003&0.8142&0.8508&1000&0.1309\\
PDF&psfgalex&O2&mean&no&SimpleWF&0.5752&0.7567&0.8731&0.9135&530&0.0694
     \enddata
     \tablecomments{The simple weightfunction is based on the SDSS+GALEX input sample of 7642 quasars.} 
     \end{deluxetable}
     
          
     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $2.1} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{Photometric Redshift Estimates for low-redshift quasars: Comparison between using 4 colors and 5 colors for quasars with GALEX matches.  \label{sdssGalex_lowtable}}
     \startdata
$\chi^2$&psf&O2&mean&no&N/A&0.5036&0.7009&0.8152&0.8495\\
PDF&psf&O2&mean&no&SimpleWF&0.5647&0.7569&0.8767&0.9162\\
$\chi^2$&psfgalex&O2&mean&no&N/A&0.5142&0.7117&0.8245&0.8580\\
PDF&psfgalex&O2&mean&no&SimpleWF&0.5871&0.7700&0.8884&0.9284
     \enddata
     \end{deluxetable}
     
     \begin{deluxetable}{c c c c c c || c c c c }
     \tablecolumns{10}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{6}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $2.1} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{Photometric Redshift Estimates for high-redshift quasars: Comparison between using 4 colors and 5 colors for quasars with GALEX matches.  \label{sdssGalex_hightable}}
     \startdata
$\chi^2$&psf&O2&mean&no&N/A&0.1747&0.2707&0.3930&0.5415\\
PDF&psf&O2&mean&no&SimpleWF&0.1834&0.2882&0.3493&0.3886\\
$\chi^2$&psfgalex&O2&mean&no&N/A&0.2052&0.3319&0.4803&0.6201\\
PDF&psfgalex&O2&mean&no&SimpleWF&0.1921&0.3275&0.3755&0.4323
     \enddata
     \end{deluxetable}    

     \begin{deluxetable}{c c c c c c c c || c c c c | c c | c c | c c | c }
     \rotate
     \tablecolumns{19}
     \tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{8}{c}{CZR Info} & \multicolumn{4}{c}{All} & \multicolumn{7}{c}{Catastrophic Failures} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{CZR errlim} &
     \colhead{z$_{phot}$ errlim} &
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$} & 
     \colhead{\# CF} & 
     \colhead{\% CF} & 
     \colhead{\# Common} & 
     \colhead{\%} &
     \colhead{\# Diff} & 
     \colhead{\%} & 
     \colhead{\# not CF}}
     \tablecaption{PDF Photometric Redshift Estimates varying magnitude error limits and removing reddened quasars.  \label{PDFvaryerror}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&10.0&10.0&0.3835&0.5889&0.7648&0.8232&6821&0.1469&NA&NA&NA&NA&NA\\
\cline{1-19}
PDF&psf&O2&mean&yes&SimpleWF&1.0&1.0&0.3982&0.5973&0.7646&0.8227&6774&0.1478&5847&0.8632&433&0.0639&974\\
PDF&psf&O2&mean&yes&SimpleWF&0.5&0.5&0.4081&0.6049&0.7639&0.8164&6935&0.1564&5407&0.7797&1030&0.1485&1414\\
PDF&psf&O2&mean&yes&SimpleWF&0.2&0.2&0.4125&0.6071&0.7629&0.8166&6743&0.1560&5123&0.7598&1133&0.1680&1698\\
PDF&psf&O2&mean&yes&SimpleWF&0.1&0.1&0.4222&0.6167&0.7642&0.8157&6169&0.1588&4460&0.7230&1281&0.2077&2361\\
PDF&psf&O2&mean&yes&SimpleWF&0.05&0.05&0.4460&0.6349&0.7741&0.8238&3881&0.1547&2635&0.6789&915&0.2358&4186\\
PDF&psf&O2&mean&yes&SimpleWF&0.02&0.02&0.4987&0.6297&0.7481&0.7935&70&0.1763&43&0.6143&27&0.3857&6778\\
\cline{1-19}
PDF&psf&C&mean&yes&SimpleWF&1.0&1.0&0.4070&0.6099&0.7707&0.8255&6463&0.1410&4996&0.7730&1000&0.1547&1825\\
PDF&psf&C&mean&yes&SimpleWF&0.5&0.5&0.4108&0.6093&0.7663&0.8187&6730&0.1517&4802&0.7135&1428&0.2122&2019\\
PDF&psf&C&mean&yes&SimpleWF&0.2&0.2&0.4153&0.6134&0.7673&0.8188&6578&0.1522&4541&0.6903&1555&0.2364&2280\\
PDF&psf&C&mean&yes&SimpleWF&0.1&0.1&0.4273&0.6252&0.7707&0.8211&5874&0.1512&3980&0.6776&1474&0.2509&2841\\
\cline{1-19}
PDF&psf&O2&mean&yes&SimpleWF&1.0&10.0&0.3964&0.5953&0.7642&0.8230&6838&0.1473&5903&0.8633&437&0.0639&918\\
PDF&psf&O2&mean&yes&SimpleWF&0.5&10.0&0.4006&0.5980&0.7623&0.8175&7149&0.1540&5590&0.7819&1049&0.1467&1231\\
PDF&psf&O2&mean&yes&SimpleWF&0.2&10.0&0.3971&0.5892&0.7496&0.8088&7390&0.1592&5533&0.7487&1325&0.1793&1288\\
PDF&psf&O2&mean&yes&SimpleWF&0.1&10.0&0.3916&0.5807&0.7392&0.7994&7736&0.1667&5482&0.7086&1691&0.2186&1339\\
PDF&psf&O2&mean&yes&SimpleWF&0.05&10.0&0.3856&0.5713&0.7253&0.7860&8276&0.1783&5414&0.6542&2246&0.2714&1407\\
PDF&psf&O2&mean&yes&SimpleWF&0.02&10.0&0.3535&0.5311&0.6915&0.7578&9093&0.1959&5257&0.5781&3173&0.3489&1564\\
PDF&psf&O2&mean&yes&SimpleWF&0.01&10.0&0.2439&0.4005&0.5702&0.6542&13250&0.2854&5055&0.3815&7290&0.5502&1766\\
\cline{1-19}
PDF&psf&C&mean&yes&SimpleWF&1.0&10.0&0.4052&0.6084&0.7701&0.8255&6527&0.1406&5049&0.7736&1008&0.1544&1772\\
PDF&psf&C&mean&yes&SimpleWF&0.5&10.0&0.4036&0.6029&0.7641&0.8189&6965&0.1500&4980&0.7150&1472&0.2113&1841\\
PDF&psf&C&mean&yes&SimpleWF&0.2&10.0&0.4006&0.5969&0.7562&0.8119&7192&0.1549&4945&0.6876&1721&0.2393&1876\\
PDF&psf&C&mean&yes&SimpleWF&0.1&10.0&0.3983&0.5932&0.7513&0.8078&7315&0.1576&4941&0.6755&1832&0.2504&1880
     \enddata
     \end{deluxetable}     


     \begin{deluxetable}{c c c c c c c c || c c c c }
     \tablecolumns{12}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{8}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{CZR errlim} &
     \colhead{z$_{phot}$ errlim} &
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for low-redshift quasars varying magnitude error limits and removing reddened quasars. \label{PDFvaryerrorlowtable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&10.0&10.0&0.3947&0.6036&0.7689&0.8196\\
\cline{1-12}
PDF&psf&O2&mean&yes&SimpleWF&1.0&1.0&0.4119&0.6131&0.7675&0.8178\\
PDF&psf&O2&mean&yes&SimpleWF&0.5&0.5&0.4169&0.6159&0.7660&0.8122\\
PDF&psf&O2&mean&yes&SimpleWF&0.2&0.2&0.4217&0.6197&0.7679&0.8143\\
PDF&psf&O2&mean&yes&SimpleWF&0.1&0.1&0.4300&0.6284&0.7698&0.8138\\
PDF&psf&O2&mean&yes&SimpleWF&0.05&0.05&0.4529&0.6454&0.7773&0.8180\\
PDF&psf&O2&mean&yes&SimpleWF&0.02&0.02&0.5013&0.6354&0.7453&0.7909\\
\cline{1-12}
PDF&psf&C&mean&yes&SimpleWF&1.0&1.0&0.4262&0.6229&0.7734&0.8199\\
PDF&psf&C&mean&yes&SimpleWF&0.5&0.5&0.4261&0.6181&0.7664&0.8123\\
PDF&psf&C&mean&yes&SimpleWF&0.2&0.2&0.4287&0.6209&0.7684&0.8138\\
PDF&psf&C&mean&yes&SimpleWF&0.1&0.1&0.4384&0.6309&0.7719&0.8169\\
\cline{1-12}
PDF&psf&O2&mean&yes&SimpleWF&1.0&10.0&0.4116&0.6126&0.7669&0.8172\\
PDF&psf&O2&mean&yes&SimpleWF&0.5&10.0&0.4158&0.6143&0.7640&0.8101\\
PDF&psf&O2&mean&yes&SimpleWF&0.2&10.0&0.4180&0.6144&0.7614&0.8076\\
PDF&psf&O2&mean&yes&SimpleWF&0.1&10.0&0.4161&0.6131&0.7578&0.8027\\
PDF&psf&O2&mean&yes&SimpleWF&0.05&10.0&0.4124&0.6073&0.7505&0.7960\\
PDF&psf&O2&mean&yes&SimpleWF&0.02&10.0&0.3854&0.5741&0.7269&0.7740\\
PDF&psf&O2&mean&yes&SimpleWF&0.01&10.0&0.2664&0.4386&0.6160&0.6931\\
\cline{1-12}
PDF&psf&C&mean&yes&SimpleWF&1.0&10.0&0.4259&0.6223&0.7727&0.8191\\
PDF&psf&C&mean&yes&SimpleWF&0.5&10.0&0.4250&0.6164&0.7642&0.8101\\
PDF&psf&C&mean&yes&SimpleWF&0.2&10.0&0.4246&0.6151&0.7616&0.8069\\
PDF&psf&C&mean&yes&SimpleWF&0.1&10.0&0.4232&0.6139&0.7581&0.8038
     \enddata
     \end{deluxetable}     

     \begin{deluxetable}{c c c c c c c c || c c c c }
     \tablecolumns{12}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{8}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{CZR errlim} &
     \colhead{z$_{phot}$ errlim} &
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for high-redshift quasars varying magnitude error limits and removing reddened quasars. \label{PDFvaryerrorhightable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&10.0&10.0&0.3947&0.6036&0.7689&0.8196\\
\cline{1-12}
PDF&psf&O2&mean&yes&SimpleWF&1.0&1.0&0.3284&0.5164&0.7496&0.8478\\
PDF&psf&O2&mean&yes&SimpleWF&0.5&0.5&0.3531&0.5361&0.7505&0.8426\\
PDF&psf&O2&mean&yes&SimpleWF&0.2&0.2&0.3468&0.5171&0.7276&0.8335\\
PDF&psf&O2&mean&yes&SimpleWF&0.1&0.1&0.3579&0.5190&0.7172&0.8317\\
PDF&psf&O2&mean&yes&SimpleWF&0.05&0.05&0.3881&0.5474&0.7468&0.8725\\
PDF&psf&O2&mean&yes&SimpleWF&0.02&0.02&0.4583&0.5417&0.7917&0.8333\\
\cline{1-12}
PDF&psf&C&mean&yes&SimpleWF&1.0&1.0&0.2677&0.5159&0.7513&0.8655\\
PDF&psf&C&mean&yes&SimpleWF&0.5&0.5&0.2633&0.5247&0.7652&0.8799\\
PDF&psf&C&mean&yes&SimpleWF&0.2&0.2&0.2583&0.5251&0.7550&0.8781\\
PDF&psf&C&mean&yes&SimpleWF&0.1&0.1&0.2604&0.5405&0.7528&0.8830\\
\cline{1-12}
PDF&psf&O2&mean&yes&SimpleWF&1.0&10.0&0.3242&0.5127&0.7516&0.8507\\
PDF&psf&O2&mean&yes&SimpleWF&0.5&10.0&0.3283&0.5205&0.7543&0.8531\\
PDF&psf&O2&mean&yes&SimpleWF&0.2&10.0&0.2979&0.4695&0.6935&0.8143\\
PDF&psf&O2&mean&yes&SimpleWF&0.1&10.0&0.2749&0.4270&0.6505&0.7835\\
PDF&psf&O2&mean&yes&SimpleWF&0.05&10.0&0.2582&0.4000&0.6056&0.7387\\
PDF&psf&O2&mean&yes&SimpleWF&0.02&10.0&0.2017&0.3265&0.5232&0.6808\\
PDF&psf&O2&mean&yes&SimpleWF&0.01&10.0&0.1368&0.2193&0.3529&0.4693\\
\cline{1-12}
PDF&psf&C&mean&yes&SimpleWF&1.0&10.0&0.2691&0.5161&0.7535&0.8676\\
PDF&psf&C&mean&yes&SimpleWF&0.5&10.0&0.2627&0.5143&0.7636&0.8773\\
PDF&psf&C&mean&yes&SimpleWF&0.2&10.0&0.2416&0.4763&0.7202&0.8452\\
PDF&psf&C&mean&yes&SimpleWF&0.1&10.0&0.2334&0.4567&0.7063&0.8344
     \enddata
     \end{deluxetable}     

     \begin{deluxetable}{c c c c c c c c || c c c c | c c | c c | c c | c }
     \rotate
     \tablecolumns{19}
     \tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{8}{c}{CZR Info} & \multicolumn{4}{c}{All} & \multicolumn{7}{c}{Catastrophic Failures} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{CZR Mag Lim} &
     \colhead{z$_{phot}$ Mag Lim} &
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$} & 
     \colhead{\# CF} & 
     \colhead{\% CF} & 
     \colhead{\# Common} & 
     \colhead{\%} &
     \colhead{\# Diff} & 
     \colhead{\%} & 
     \colhead{\# not CF}}
     \tablecaption{PDF Photometric Redshift Estimates varying magnitude limits and removing reddened quasars.  \label{PDFvarymags}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&None&None&0.3835&0.5889&0.7648&0.8232&6821&0.1469&NA&NA&NA&NA&NA\\
\cline{1-19}
PDF&psf&O2&mean&yes&SimpleWF&25.0&25.0&0.3898&0.5963&0.7687&0.8237&6830&0.1485&6055&0.8865&296&0.0433&766\\
PDF&psf&O2&mean&yes&SimpleWF&21.0&21.0&0.4172&0.6075&0.7567&0.8127&6839&0.1619&4809&0.7032&1572&0.2299&2012\\
PDF&psf&O2&mean&yes&SimpleWF&20.0&20.0&0.4545&0.6505&0.7945&0.8486&4471&0.1296&3148&0.7041&982&0.2196&3673\\
\cline{1-19}
PDF&psf&C&mean&yes&SimpleWF&25.0&25.0&0.3975&0.6074&0.7712&0.8260&6539&0.1422&5121&0.7831&952&0.1456&1700\\
PDF&psf&C&mean&yes&SimpleWF&21.0&21.0&0.4263&0.6218&0.7735&0.8252&6228&0.1474&4239&0.6806&1556&0.2498&2582\\
PDF&psf&C&mean&yes&SimpleWF&20.0&20.0&0.4615&0.6634&0.8050&0.8531&4287&0.1243&2852&0.6653&1108&0.2585&3969\\
\cline{1-19}
PDF&psf&O2&mean&yes&SimpleWF&25.0&None&0.3882&0.5948&0.7683&0.8243&6857&0.1477&6080&0.8867&296&0.0432&741\\
PDF&psf&O2&mean&yes&SimpleWF&21.0&None&0.3890&0.5700&0.7222&0.7861&8227&0.1772&5371&0.6529&2252&0.2737&1450\\
PDF&psf&O2&mean&yes&SimpleWF&20.0&None&0.3904&0.5719&0.7156&0.7754&8907&0.1919&5099&0.5725&3179&0.3569&1722\\
\cline{1-19}
PDF&psf&C&mean&yes&SimpleWF&25.0&None&0.3962&0.6064&0.7711&0.8265&6566&0.1415&5144&0.7834&954&0.1453&1677\\
PDF&psf&C&mean&yes&SimpleWF&21.0&None&0.3971&0.5834&0.7375&0.7940&8082&0.1741&4770&0.5902&2717&0.3362&2051\\
PDF&psf&C&mean&yes&SimpleWF&20.0&None&0.4007&0.5888&0.7336&0.7855&8596&0.1852&4705&0.5473&3288&0.3825&2116
     \enddata
     \end{deluxetable}     


     \begin{deluxetable}{c c c c c c c c || c c c c }
     %\rotate
     \tablecolumns{12}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{8}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{CZR Mag Lim} &
     \colhead{z$_{phot}$ Mag Lim} &
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for low-redshift quasars varying magnitude limits and removing reddened quasars. \label{PDFvarymagslowtable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&None&None&0.3947&0.6036&0.7689&0.8196\\
\cline{1-12}          
PDF&psf&O2&mean&yes&SimpleWF&25.0&25.0&0.3977&0.6068&0.7699&0.8181\\
PDF&psf&O2&mean&yes&SimpleWF&21.0&21.0&0.4287&0.6238&0.7670&0.8141\\
PDF&psf&O2&mean&yes&SimpleWF&20.0&20.0&0.4634&0.6636&0.8021&0.8482\\
\cline{1-12}
PDF&psf&C&mean&yes&SimpleWF&25.0&25.0&0.4158&0.6191&0.7725&0.8189\\
PDF&psf&C&mean&yes&SimpleWF&21.0&21.0&0.4373&0.6267&0.7741&0.8218\\
PDF&psf&C&mean&yes&SimpleWF&20.0&20.0&0.4706&0.6666&0.8049&0.8501\\
\cline{1-12}
PDF&psf&O2&mean&yes&SimpleWF&25.0&None&0.3976&0.6066&0.7697&0.8178\\
PDF&psf&O2&mean&yes&SimpleWF&21.0&None&0.4222&0.6144&0.7558&0.8026\\
PDF&psf&O2&mean&yes&SimpleWF&20.0&None&0.4286&0.6253&0.7656&0.8132\\
\cline{1-12}
PDF&psf&C&mean&yes&SimpleWF&25.0&None&0.4156&0.6189&0.7722&0.8186\\
PDF&psf&C&mean&yes&SimpleWF&21.0&None&0.4306&0.6175&0.7633&0.8109\\
PDF&psf&C&mean&yes&SimpleWF&20.0&None&0.4348&0.6252&0.7654&0.8125
     \enddata
     \end{deluxetable}     

     \begin{deluxetable}{c c c c c c c c || c c c c }
     %\rotate
     \tablecolumns{12}
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{8}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{CZR Mag Lim} &
     \colhead{z$_{phot}$ Mag Lim} &
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for high-redshift quasars varying magnitude limits and removing reddened quasars. \label{PDFvarymagshightable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&None&None&0.3947&0.6036&0.7689&0.8196\\
\cline{1-12}
PDF&psf&O2&mean&yes&SimpleWF&25.0&25.0&0.3502&0.5437&0.7625&0.8517\\
PDF&psf&O2&mean&yes&SimpleWF&21.0&21.0&0.3208&0.4715&0.6710&0.8011\\
PDF&psf&O2&mean&yes&SimpleWF&20.0&20.0&0.3669&0.5206&0.7189&0.8520\\
\cline{1-12}
PDF&psf&C&mean&yes&SimpleWF&25.0&25.0&0.2679&0.5238&0.7627&0.8769\\
PDF&psf&C&mean&yes&SimpleWF&21.0&21.0&0.2598&0.5473&0.7648&0.8762\\
PDF&psf&C&mean&yes&SimpleWF&20.0&20.0&0.2873&0.6016&0.8073&0.9113\\
\cline{1-12}
PDF&psf&O2&mean&yes&SimpleWF&25.0&None&0.3437&0.5385&0.7621&0.8549\\
PDF&psf&O2&mean&yes&SimpleWF&21.0&None&0.2310&0.3589&0.5626&0.7072\\
PDF&psf&O2&mean&yes&SimpleWF&20.0&None&0.2085&0.3182&0.4776&0.5956\\
\cline{1-12}
PDF&psf&C&mean&yes&SimpleWF&25.0&None&0.2681&0.5238&0.7641&0.8785\\
PDF&psf&C&mean&yes&SimpleWF&21.0&None&0.1758&0.3577&0.5667&0.6822\\
PDF&psf&C&mean&yes&SimpleWF&20.0&None&0.1754&0.3487&0.5233&0.6066
     \enddata
     \end{deluxetable}     

     \begin{deluxetable}{c c c c c c c || c c c c | c c | c c | c c | c }
     \rotate
     \tablecolumns{18}
     \tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{7}{c}{CZR Info} & \multicolumn{4}{c}{All} & \multicolumn{7}{c}{Catastrophic Failures} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{Mag Bins} &
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$} & 
     \colhead{\# CF} & 
     \colhead{\% CF} & 
     \colhead{\# Common} & 
     \colhead{\%} &
     \colhead{\# Diff} & 
     \colhead{\%} & 
     \colhead{\# not CF}}
     \tablecaption{PDF Photometric Redshift Estimates using other weighting functions.  \label{PDFapparMagWFtable}}
     \startdata
 PDF&psf&O2&mean&yes&SimpleWF&NA&0.3835&0.5889&0.7648&0.8232&6821&0.1469&NA&NA&NA&NA&NA\\
 PDF&psf&O2&mean&yes&NoWF&NA&0.3871&0.5890&0.7502&0.8074&7481&0.1612&4831&0.6458&2650&0.3542&1990\\
 \cline{1-18}
 PDF&psf&O2&mean&yes&apparMagWF&sdssdr3\_1.0&0.3930&0.5970&0.7703&0.8297&6524&0.1405&5493&0.8420&574&0.0880&1328\\
PDF&psf&O2&mean&yes&apparMagWF&sdssdr3\_0.5&0.3973&0.5984&0.7720&0.8322&6401&0.1379&5367&0.8385&587&0.0917&1454\\     
PDF&psf&O2&mean&yes&apparMagWF&sdssdr3\_5bins&0.3940&0.5957&0.7697&0.8301&6498&0.1400&5456&0.8396&579&0.0891&1365\\
\cline{1-18}

PDF&psf&O2&mean&yes&NofMfromfile&sdssdr3\_abs0.5&0.3452&0.5436&0.7124&0.7758&8842&0.1905&4963&0.5613&3255&0.3681&1858\\ 
PDF&psf&O2&mean&yes&collapsedmatrixNofz&sdssdr3\_abs0.5&0.2208&0.3606&0.5263&0.6038&16600&0.3576&5113&0.3080&10275&0.6190&1708\\
PDF&psf&O2&mean&yes&matrixNofz&sdssdr3\_abs0.5&0.3628&0.5625&0.7397&0.8068&7255&0.1563&4144&0.5712&3111&0.4288&2677
\enddata
\end{deluxetable}

     \begin{deluxetable}{c c c c c c c || c c c c }
     \tablecolumns{11}
     %\rotate
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{7}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{Mag Bins} &
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for low-redshift quasars using other weighting functions.  \label{PDFapparMagWF_lowtable}}
     \startdata
     PDF&psf&O2&mean&yes&SimpleWF&NA&0.3947&0.6036&0.7689&0.8196\\
     PDF&psf&O2&mean&yes&NoWF&NA&0.4105&0.6142&0.7657&0.8173\\
\cline{1-11}
PDF&psf&O2&mean&yes&apparMagWF&sdssdr3\_1.0&0.4058&0.6135&0.7757&0.8273\\
PDF&psf&O2&mean&yes&apparMagWF&sdssdr3\_0.5&0.4099&0.6145&0.7777&0.8301\\
PDF&psf&O2&mean&yes&apparMagWF&sdssdr3\_5bins&0.4065&0.6118&0.7753&0.8278\\
\cline{1-11}
PDF&psf&O2&mean&yes&NofMfromfile&sdssdr3\_abs0.5&0.3457&0.5408&0.6987&0.7550\\ 
PDF&psf&O2&mean&yes&collapsedmatrixNofz&sdssdr3\_abs0.5&0.1991&0.3320&0.4807&0.5419\\
PDF&psf&O2&mean&yes&matrixNofz&sdssdr3\_abs0.5&0.3941&0.6063&0.7769&0.8327\\
\enddata
\end{deluxetable}

     \begin{deluxetable}{c c c c c c c || c c c c }
     \tablecolumns{11}
     %\rotate
     %\tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{7}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $division2} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{Mag Bins} &
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$}}
     \tablecaption{PDF Photometric Redshift Estimates for high-redshift quasars using other weighting functions.  \label{PDFapparMagWF_hightable}}
     \startdata
PDF&psf&O2&mean&yes&SimpleWF&NA&0.3303&0.5189&0.7458&0.8403\\
PDF&psf&O2&mean&yes&NoWF&NA&0.2762&0.4692&0.6767&0.7601\\
\cline{1-11}
PDF&psf&O2&mean&yes&apparMagWF&sdssdr3\_1.0&0.3322&0.5186&0.7450&0.8412\\
PDF&psf&O2&mean&yes&apparMagWF&sdssdr3\_0.5&0.3370&0.5217&0.7450&0.8425\\
PDF&psf&O2&mean&yes&apparMagWF&sdssdr3\_5bins&0.3349&0.5191&0.7433&0.8410\\
\cline{1-11}
PDF&psf&O2&mean&yes&NofMfromfile&sdssdr3\_0.5&0.3428&0.5571&0.7777&0.8744\\
PDF&psf&O2&mean&yes&collapsedmatrixNofz&sdssdr3\_abs0.5&0.3239&0.4961&0.7427&0.8980\\
PDF&psf&O2&mean&yes&matrixNofz&sdssdr3\_abs0.5&0.2142&0.3546&0.5628&0.6837\\
\enddata
\end{deluxetable}

    
     \clearpage
     
     \begin{deluxetable}{c c c c c c c || c c c c || c c}
     \tablecolumns{13}
     %\tabletypesize{\scriptsize}
     \tablehead{
     \multicolumn{7}{c}{CZR Info} & \multicolumn{6}{c}{All} \\
     \colhead{Subpop} &
     \colhead{Type} &
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} &
     \colhead{$<0.05$} &
     \colhead{$<0.1$} &
     \colhead{$<0.2$} &
     \colhead{$<0.3$} &
     \colhead{CF} &
     \colhead{$\%$ CF}
     }
     \tablecaption{Photometric Redshift Estimates for subpopulations in the SDSS DR3 Quasar Catalog. \label{sdsssubpops_alltable}}
    \startdata
    extended&PDF&psf&O2&mean&no&NoWF&0.4295&0.5441&0.5778&0.5922&788&0.3794\\
radio&PDF&psf&O2&mean&no&NoWF&0.3301&0.5134&0.6678&0.7397&832&0.2215\\
IR&PDF&psf&O2&mean&no&NoWF&0.4850&0.6387&0.7523&0.7925&1158&0.1870\\
xray&PDF&psf&O2&mean&no&NoWF&0.5314&0.6849&0.7590&0.7844&525&0.1965\\
BALs&PDF&psf&O2&mean&no&NoWF&0.2121&0.3229&0.4455&0.5089&953&0.4142\\
     \cline{1-13}
extended&PDF&psf&O2&mean&no&SimpleWF&0.6769&0.8604&0.9100&0.9292&103&0.0496\\
radio&PDF&psf&O2&mean&no&SimpleWF&0.3261&0.5023&0.6753&0.7501&788&0.2097\\
IR&PDF&psf&O2&mean&no&SimpleWF&0.5276&0.6755&0.7784&0.8178&1021&0.1649\\
xray&PDF&psf&O2&mean&no&SimpleWF&0.6261&0.7897&0.8589&0.8870&230&0.0861\\
BALs&PDF&psf&O2&mean&no&SimpleWF&0.2399&0.3855&0.5554&0.6367&725&0.3151\\
red&PDF&psf&O2&mean&no&SimpleWF&0.2346&0.4009&0.6398&0.7257&641&0.2313
    \enddata
    \end{deluxetable}

\begin{deluxetable}{c c c c c c c || c c c c }
     \tablecolumns{11}
     %\tabletypesize{\scriptsize}
     \tablehead{
     \multicolumn{7}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $2.1} \\
     \colhead{Subpop} &
     \colhead{Type} &
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} &
     \colhead{$<0.05$} &
     \colhead{$<0.1$} &
     \colhead{$<0.2$} &
     \colhead{$<0.3$}}
     \tablecaption{Photometric Redshift Estimates for low-redshift quasars in subpopulations in the SDSS DR3 Quasar Catalog.  \label{sdsssubpops_lowtable}}
     \startdata
     extended&PDF&psf&O2&mean&no&NoWF&0.4332&0.5468&0.5780&0.5898\\
radio&PDF&psf&O2&mean&no&NoWF&0.3621&0.5477&0.6878&0.7585\\
IR&PDF&psf&O2&mean&no&NoWF&0.5246&0.6808&0.7875&0.8249\\
xray&PDF&psf&O2&mean&no&NoWF&0.5355&0.6883&0.7602&0.7830\\
BALs&PDF&psf&O2&mean&no&NoWF&0.2593&0.3882&0.5165&0.5834\\
     \cline{1-11}
     extended&PDF&psf&O2&mean&no&SimpleWF&0.6839&0.8688&0.9171&0.9351\\
radio&PDF&psf&O2&mean&no&SimpleWF&0.3499&0.5273&0.6782&0.7397\\
IR&PDF&psf&O2&mean&no&SimpleWF&0.5741&0.7279&0.8218&0.8557\\
xray&PDF&psf&O2&mean&no&SimpleWF&0.6344&0.7986&0.8677&0.8951\\
BALs&PDF&psf&O2&mean&no&SimpleWF&0.2398&0.3859&0.5633&0.6392\\
red&PDF&psf&O2&mean&no&SimpleWF&0.2351&0.3663&0.5743&0.6590
     \enddata
     \end{deluxetable}
    

      \begin{deluxetable}{c c c c c c c || c c c c }
     \tablecolumns{11}
     %\tabletypesize{\scriptsize}
     \tablehead{
     \multicolumn{7}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $2.1} \\
     \colhead{Subpop} &
     \colhead{Type} &
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} &
     \colhead{$<0.05$} &
     \colhead{$<0.1$} &
     \colhead{$<0.2$} &
     \colhead{$<0.3$}}
     \tablecaption{Photometric Redshift Estimates for high-redshift quasars in subpopulations in the SDSS DR3 Quasar Catalog.  \label{sdsssubpops_hightable}}
     \startdata
extended&PDF&psf&O2&mean&no&NoWF&0.1481&0.3333&0.5556&0.7778\\
radio&PDF&psf&O2&mean&no&NoWF&0.1973&0.3712&0.5849&0.6616\\
IR&PDF&psf&O2&mean&no&NoWF&0.1386&0.2709&0.4441&0.5087\\
xray&PDF&psf&O2&mean&no&NoWF&0.2683&0.4634&0.6829&0.8780\\
BALs&PDF&psf&O2&mean&no&NoWF&0.0453&0.0925&0.1949&0.2461\\
     \cline{1-11}
extended&PDF&psf&O2&mean&no&SimpleWF&0.1481&0.2222&0.3704&0.4815\\
radio&PDF&psf&O2&mean&no&SimpleWF&0.2274&0.3986&0.6630&0.7932\\
IR&PDF&psf&O2&mean&no&SimpleWF&0.1213&0.2173&0.3984&0.4866\\
xray&PDF&psf&O2&mean&no&SimpleWF&0.0976&0.2195&0.2927&0.3659\\
BALs&PDF&psf&O2&mean&no&SimpleWF&0.2402&0.3839&0.5276&0.6280\\
red&PDF&psf&O2&mean&no&SimpleWF&0.2338&0.4494&0.7316&0.8190
     \enddata
     \end{deluxetable}

     \begin{deluxetable}{c c c c c c c || c c c c | c c | c c | c c | c }
     \rotate
     \tablecolumns{18}
     \tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{7}{c}{CZR Info} & \multicolumn{4}{c}{All} & \multicolumn{7}{c}{Catastrophic Failures} \\
     \colhead{Type} & 
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Corr?} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$<0.05$} & 
     \colhead{$<0.1$} & 
     \colhead{$<0.2$} & 
     \colhead{$<0.3$} & 
     \colhead{CF} & 
     \colhead{\% CF} & 
     \colhead{Common} & 
     \colhead{\%} &
     \colhead{Diff} & 
     \colhead{\%} & 
     \colhead{not CF}}
     \tablecaption{PDF Photometric Redshift Estimates for quasars in the SDSS DR3 Quasar Catalog including correlation.   \label{corr_alltable}}
     \startdata
PDF&psf&O2&mean&no&yes&SimpleWF&0.3835&0.5889&0.7648&0.8232&6821&0.1469&NA&NA&NA&NA&NA\\
PDF&psf&O2&gmedian&no&yes&SimpleWF&0.3787&0.5840&0.7577&0.8193&6933&0.1494&6062&0.8744&382&0.0551&759\\
PDF&psf&O2&gmode&no&yes&SimpleWF&0.3675&0.5696&0.7451&0.8105&7224&0.1556&5795&0.8022&924&0.1279&1026\\
\cline{1-17}
PDF&psf&O2&mean&yes&yes&SimpleWF&0.3837&0.5892&0.7650&0.8237&6784&0.1461&6258&0.9225&43&0.0063&563\\   
PDF&psf&O2&gmedian&yes&yes&SimpleWF&0.3797&0.5848&0.7584&0.8197&6907&0.1488&6053&0.8764&369&0.0534&768\\   
PDF&psf&O2&gmode&yes&yes&SimpleWF&0.3688&0.5684&0.7443&0.8098&7237&0.1559&5794&0.8006&934&0.1291&1027
    \enddata
    \end{deluxetable}


     \begin{deluxetable}{c c c c c c c || c c c c }
     \tablecolumns{11}
     %\tabletypesize{\scriptsize}
     \tablehead{
     \multicolumn{7}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}\leq $2.1} \\
     \colhead{Type} &
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Corr?} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} &
     \colhead{$<0.05$} &
     \colhead{$<0.1$} &
     \colhead{$<0.2$} &
     \colhead{$<0.3$}}
     \tablecaption{Photometric Redshift Estimates for low-redshift quasars in the SDSS DR3 Quasar Catalog including correlation.  \label{corr_lowtable}}
     \startdata
     PDF&psf&O2&mean&no&yes&SimpleWF&0.3947&0.6036&0.7689&0.8196\\
     PDF&psf&O2&gmedian&no&yes&SimpleWF&0.3899&0.5982&0.7614&0.8157\\
     PDF&psf&O2&gmode&no&yes&SimpleWF&0.3745&0.5808&0.7469&0.8026\\
     \cline{1-11}
     PDF&psf&O2&mean&yes&yes&SimpleWF&0.3951&0.6040&0.7693&0.8205\\   
PDF&psf&O2&gmedian&yes&yes&SimpleWF&0.3913&0.5995&0.7624&0.8165\\   
PDF&psf&O2&gmode&yes&yes&SimpleWF&0.3772&0.5806&0.7465&0.8023
     \enddata
     \end{deluxetable}
     
     \begin{deluxetable}{c c c c c c c || c c c c }
     \tablecolumns{11}
     %\tabletypesize{\scriptsize}
     \tablehead{
     \multicolumn{7}{c}{CZR Info} & \multicolumn{4}{c}{$z_{spec}> $2.1} \\
     \colhead{Type} &
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Corr?} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} &
     \colhead{$<0.05$} &
     \colhead{$<0.1$} &
     \colhead{$<0.2$} &
     \colhead{$<0.3$}}
     \tablecaption{Photometric Redshift Estimates for high-redshift quasars in the SDSS DR3 Quasar Catalog including correlation.  \label{corr_hightable}}
     \startdata
     PDF&psf&O2&mean&no&yes&SimpleWF&0.3303&0.5189&0.7458&0.8403\\
     PDF&psf&O2&gmedian&no&yes&SimpleWF&0.3255&0.5165&0.7399&0.8367\\
     PDF&psf&O2&gmode&no&yes&SimpleWF&0.3342&0.5167&0.7367&0.8482\\
     \cline{1-11}
     PDF&psf&O2&mean&yes&yes&SimpleWF&0.3296&0.5191&0.7445&0.8392\\
PDF&psf&O2&gmedian&yes&yes&SimpleWF&0.3245&0.5154&0.7394&0.8350\\
PDF&psf&O2&gmode&yes&yes&SimpleWF&0.3287&0.5105&0.7337&0.8454
     \enddata
     \end{deluxetable}
     
     \clearpage
     
          \begin{deluxetable}{c c c c c | c c c | c c c | c c c | c c c }
     \tablecolumns{17}
     \rotate
     \tabletypesize{\scriptsize}
     \tablehead{ 
     \multicolumn{5}{c}{Info} & \multicolumn{3}{c}{All} & \multicolumn{3}{c}{no CF} &\multicolumn{3}{c}{$z_{spec}\leq $2.1} &\multicolumn{2}{c}{$z_{spec}> $2.1} \\
     \colhead{Mag} &
     \colhead{Bins} &
     \colhead{Stat} &
     \colhead{Red Rem.?} &
     \colhead{Weighting} & 
     \colhead{$\Delta$z} &
     \colhead{$\Delta$z/(1+z)} &
     \colhead{$\Delta$z$^2$} &
     \colhead{$\Delta$z} &
     \colhead{$\Delta$z/(1+z)} &
     \colhead{$\Delta$z$^2$} &
     \colhead{$\Delta$z} &
     \colhead{$\Delta$z/(1+z)} &
     \colhead{$\Delta$z$^2$} &
     \colhead{$\Delta$z} &
     \colhead{$\Delta$z/(1+z)} &
     \colhead{$\Delta$z$^2$} }
     \tablecaption{Mean Statistics for selected variations for calculating PDF PhotoZs.  \label{otherstats}}
     \startdata
psf&O2&mean&yes&SimpleWF&0.2830&0.1392&0.3466&0.0864&0.0342&0.0150&0.2859&0.1523&0.3567&0.2694&0.0772&0.2984\\
psf&C&mean&yes&SimpleWF&0.2686&0.1258&0.3176&0.0849&0.0339&0.0150&0.2720&0.1347&0.3278&0.2457&0.0667&0.2500\\
psf&E&mean&yes&SimpleWF&0.2695&0.1289&0.3188&0.0861&0.0341&0.0154&0.2824&0.1411&0.3456&0.1843&0.0486&0.1418\\
model&O2&mean&yes&SimpleWF&0.2755&0.1325&0.3334&0.0846&0.0334&0.0146&0.2757&0.1439&0.3385&0.2742&0.0786&0.3094\\
model&C&mean&yes&SimpleWF&0.2617&0.1199&0.3048&0.0832&0.0332&0.0145&0.2643&0.1281&0.3131&0.2445&0.0662&0.2500\\
model&E&mean&yes&SimpleWF&0.2607&0.1220&0.3028&0.0840&0.0333&0.0149&0.2722&0.1331&0.3268&0.1848&0.0487&0.1442\\
psf&O2&mean&no&SimpleWF&0.2774&0.1345&0.3190&0.0889&0.0350&0.0153&0.2561&0.1398&0.2839&0.3790&0.1092&0.4858\\
psf&C&mean&no&SimpleWF&0.2776&0.1251&0.3118&0.0894&0.0359&0.0159&0.2688&0.1300&0.2967&0.3359&0.0925&0.4116\\
model&G&mean&no&SimpleWF&0.2534&0.1204&0.2756&0.0866&0.0340&0.0154&0.2654&0.1318&0.2989&0.1738&0.0452&0.1214
     \enddata
     \end{deluxetable}

%     \begin{deluxetable}{c c c c c c c || c c c c | c c | c c | c c | c }
 %  \rotate
%     \tablecolumns{18}
%     \tabletypesize{\scriptsize}
%     \tablehead{ 
%     \multicolumn{7}{c}{CZR Info} & \multicolumn{4}{c}{All} & \multicolumn{7}{c}{Catastrophic Failures} \\
%     \colhead{mBin} & 
%     \colhead{vary} &
%     \colhead{Mag} &
%     \colhead{Bins} &
%     \colhead{Stat} &
%     \colhead{Red Rem.?} &
%     \colhead{Weighting} & 
%     \colhead{$<0.05$} & 
%     \colhead{$<0.1$} & 
%     \colhead{$<0.2$} & 
%     \colhead{$<0.3$} & 
%     \colhead{\# CF} & 
%     \colhead{\% CF} & 
%     \colhead{\# Common} & 
%     \colhead{\%} &
%     \colhead{\# Diff} & 
%     \colhead{\%} & 
%     \colhead{\# not CF}}
%     \tablecaption{PDF Photometric Redshift Estimates using Luminosity Function based Weighting Function.  \label{PDFLumWFO2}}
%     \startdata
%NA&&psf&O2&mean&yes&SimpleWF&0.3115&0.4846&0.7007&0.8135\\
%\cline{1-18}
%0.5&&psf&O2&mean&yes&LumWF&0.2343&0.3564&0.4623&0.5061&21241&0.4576&5944&0.2798&13945&0.6565&3421\\
%0.5&norm&psf&O2&mean&yes&LumWF&0.2343&0.3564&0.4624&0.5061&21237&0.4575&5944&0.2799&13945&0.6566&3421\\
%0.5&nonorm&psf&O2&mean&yes&LumWF&0.2343&0.3564&0.4624&0.5061&21237&0.4575&5944&0.2799&13945&0.6566&3421\\
%0.2&norm&psf&O2&mean&yes&LumWF&0.2343&0.3564&0.4624&0.5061&21237&0.4575&5944&0.2799&13945&0.6566&3421\\
%1.0&norm&psf&O2&mean&yes&LumWF&0.2343&0.3564&0.4624&0.5061&21237&0.4575&5944&0.2799&13945&0.6566&3421
%     \enddata
%     \end{deluxetable}     



 

==> redshifttypemag.tex <==
\chapter{The Dependence on Redshift, Type, \& Broad-band Luminosity}$\footnote{Material in this chapter was originally published in \emph{The Astrophysical Journal} in November 2008 (ApJ 688:180)}$\note{figure out proper way to cite paper}

\section{OVERVIEW}
In Figure~\ref{scale_spectargs}, we present the mean cumulative overdensity of photometric galaxies as a function of scale for the QI\_pt, QII\_Z, AI, and AII spectroscopic samples.  There are clear differences: %between the environment overdensities for each of the spectroscopic target samples: 
Type II objects are in more overdense environments than Type I objects for both higher luminosity AGN (i.e. quasars) and lower luminosity AGN, and quasars are in the most overdense environments at all scales.  Within a scale of $\approx150\kpchseventy$, QII\_Zs have an environment 1.4 times more overdense than that of QI\_pts, albeit with large errors, while the AIIs have an environment 1.3 times more overdense than AIs.  At the same scale, the QI\_pts have environments more overdense than AIs by a factor of 1.8, and QII\_Zs have environments 1.9 times more overdense than AIIs.  Moving out to the scale of $\approx 1\Mpchseventy$, the QII\_Zs again have an environment 1.4 more overdense than the environment of QI\_pts, and the QI\_pts are in environments 1.4 times more overdense than AIs.  

The differences between the target samples' environment overdensities could be an effect of AGN type, however, and the intertwined effects of AGN luminosity and redshift will certainly play into these differences.  In this chapter, we explore how type, redshift and absolute magnitude influence the measured differences in AGN environments. 

\section{TARGET REDSHIFT}\label{redshiftsubsec}
We first investigate only the effects of redshift.  Figure~\ref{redshift_spectargs} shows the mean cumulative overdensity as a function of redshift for the spectroscopic target samples, which provides marginal evidence for redshift evolution in the environment overdensity of  QI\_pts.  The magenta dashed line shows the linear weighted least-squares fit to the QI\_pt environment overdensity data with redshift at different maximum radii;  the fitting parameters for these lines is given in Table~\ref{table_compareFit}. The rightmost column of the table gives the $\chi^2$ probability for each fit using the relevant degrees of freedom.  The best linear fit for the smallest scale of $R \leq0.1\Mpchseventy$ has a slope of $-1.171$, which suggests decreasing overdensity with increasing redshift, and for $R \leq0.25\Mpchseventy$, the overdensity increases with redshift: the best linear fit has a slope of $1.276$.  While these fits indicate a slight redshift dependence, we also try a zero-slope linear fit (which necessarily has one less degree of freedom than the best-fit line) and find that the zero-slope fit, i.e., no redshift dependence, is also a good fit to the data and in some cases is slightly more likely.  Higher precision and higher redshift measurements will be necessary to place strong constraints on the functional form of environment overdensity evolution with redshift.  
If the environment overdensity is indeed independent of redshift, this implies that the significant differences in environment seen in Figure~\ref{scale_spectargs} are caused primarily by luminosity and type effects, rather than the influence of redshift evolution.

In the top panel of Figure~\ref{scale_spectargs_z}, we show the evolution of the mean cumulative overdensity of photometric galaxies in the environments of QI\_pt, AI and AII samples.  It is important to recall that we have placed the random points at the same redshift as the spectroscopic targets, and that we have imposed $\delta z$ cuts on the photometric galaxies (as described in Section~\ref{deltazcutsection}) in order to minimize the effect of redshift evolution in the photometric galaxy sample.  Therefore we can compare objects in different redshift bins.  Figure~\ref{scale_spectargs_z} demonstrates that higher redshift QI\_pts are in environments 1.24 times more overdense than the lower redshift quasars on scales $\lesssim500\kpchseventy$, while at larger scales, there appears to be little-to-no redshift evolution.  However, there is scale-dependent redshift evolution evident on scales $\lesssim1.0\Mpchseventy$ for the AIIs, shown in the lowest panel.  The AIs begin to exhibit noticeable redshift evolution at scales $\lesssim300\kpchseventy$, where the environments of lower redshift AIs are 1.26 times less dense than those of the higher redshift AIs. 

We see therefore that there is some evidence for a change in local environment as a function of redshift, all else being held constant.  However, we have not yet taken AGN luminosity into account.  Even in the same redshift range, selection effects due to the magnitude-limited samples may come into play, which we investigate in Sections~\ref{absmagsubsec} and \ref{allsubsec}.  

\section{TARGET TYPE}\label{typesubsec}
In Figure~\ref{scale_spectargs_type}, we identify three redshift ranges where there is overlap between our AGN samples and explore whether differences in type are reflected in the relative overdensity.  The top panel shows the overdensity as a function of scale for both types of higher-luminosity AGNs (i.e. quasars) in the range $0.3\leq z\leq0.6$, and for both types of lower-luminosity AGNs in two redshift ranges, $0.11\leq z\leq0.15$ and $0.15<z\leq0.33$.  The dividing redshift value of $z=0.15$ is chosen to roughly equalize the number of lower-luminosity AGNs in each redshift range.  The lower three panels show the ratio of Type II environment overdensity to Type I environment overdensity in the three redshift ranges.  Again, we are able to compare objects in different redshift ranges because we have imposed $\delta z$ cuts on the photometric galaxies around both the spectroscopic targets and the random positions to which they are compared in order to account for any redshift evolution in the photometric galaxy sample and to minimize projection effects.  

QII\_Zs have higher overdensity environments than QI\_pts with little scale dependence: at $R\approx1.0\Mpchseventy$, the overdensity of QII\_Z environments is a factor of 1.4 greater than the overdensity of QI\_pt environments, and at the smaller scale of $R\approx250\kpchseventy$, the QII\_Z environments have 1.2 times the overdensity of QI\_pt environments.   However, the large errors prevent us from drawing strong conclusions.  

Type II environment overdensity is again consistently about a factor of 1.3 higher on all scales than the Type I environment overdensity for AIs and AIIs in the redshift range $0.15<z\leq0.33$.  In the lower redshift range of $0.11\leq z\leq0.15$, however, the AII and AI environment overdensities have a ratio consistent with unity until scales $R<200\kpchseventy$, where the ratio increases to 1.3.  This agrees with the work of \citet{Koulouridis}, who found that Type II Seyfert galaxies were more likely to have a close neighbor than Type I Seyferts, using small samples of Seyfert 1 and 2 galaxies at very low redshifts.

Because we see increased overdensity for AIIs compared to AIs on small scales in overlapping redshift ranges, we can conclude that in Figure~\ref{scale_spectargs}, the differences seen in environment overdensity between the AGN types are not primarily due to redshift evolution.  However, we have not ruled out the effects of AGN luminosity.  The AI and AII samples are selected from magnitude-limited spectroscopic galaxy samples, which will be dominated by intrinsically more luminous sources at higher redshift.  The AI sample could be more affected by this magnitude limit, as the broad emission lines contribute more significantly to the overall flux in a given band and therefore the two AGN populations could have different average intrinsic luminosities.  

\section{TARGET BROAD-BAND LUMINOSITY}\label{absmagsubsec}

Unlike Type I quasars, which are targeted largely based on their strong nuclear luminosity \citep{Schneider}, the lower luminosity AGN we use were selected from objects classified as galaxies by the SDSS selection algorithms \citep{Haoa}.  The broad-band flux of these sources will be dominated by host galaxy starlight and/or flux from star formation, etc., which has little or no association with the nuclear luminosity.  Therefore, we first focus on the QI\_pt sample for our analysis of the relationship between absolute magnitude and environment, as the sample spans the entire redshift range we study, and with this long redshift baseline we are best able to disentangle redshift and luminosity effects on environment overdensity.  

In order to verify that the observed evidence for evolution of environment overdensity is not due to the $i\leq19.1$ ($z \lesssim 3.0$) limit imposed on QI selection in the SDSS \citep{Schneider}, we perform several tests in which we vary the apparent magnitude limit of the data.  We consider two quasar samples limited to $i\leq18.9$ and to the $i\leq19.1$ SDSS limit.  
The two magnitude-limited samples were each then separated into two luminosity bins.  We compared environment overdensity measurements of bright or dim quasars in each of the magnitude-limited samples and found no appreciable difference.  Additionally, no difference was observed when different absolute magnitude values were used to define the bright and dim samples.  In order to ensure that there is no difference between environments of quasars with $i > 19.1$, which were selected by the high-redshift targeting algorithm, and the rest of the apparent magnitude-selected sample, we performed similar tests comparing the environment overdensity of the entire quasar sample to that of the subset of quasars with $i\leq18.9$ or $i>19.1$.  In all cases, there was no appreciable change in the observed overdensity. 

We compare the environment overdensities of QI\_pt in two luminosity bins to the other target samples without redshift cuts in Figure~\ref{scale_spectargs_M}.  The threshold value $M_{i}=-23.2$ is chosen to give roughly equal numbers of QI\_pt sources in each luminosity bin: there are 2,190 (2,044) quasars with $-27.5\leq M_{i} \leq-23.2$ ($-23.2<M_{i}\leq-22.0$).  The average magnitude of the brighter (fainter) bin is $\overline{M_{i}}=-23.83$ ($\overline{M_{i}}=-22.70$).  

QII\_Zs and the brighter QI\_pt sources are located in similarly overdense environments consistently at all scales, while the dimmer QI\_pts are located in environments slightly less overdense than the QII\_Zs.  At a scale $R\approx500\kpchseventy$, the cumulative overdensity of QII\_Z environment is 1.06 times that of the brighter QI\_pts, but 1.3 times as the dimmer QI\_pts.  At the scale of $R\approx1.0\Mpchseventy$, QII\_Zs have environment overdensities 1.2 times the environment overdensity of brighter QI\_pts but 1.5 times that of dimmer QI\_pts.  Again we note that the large error bars nearly overlap with unity and prevent strong conclusions.  

The more luminous QI\_pts are located in environments more overdense than AIs, while there is less difference in the overdensities of dimmer QI\_pts and AIs.  The environment overdensity ratio increases with decreasing scale for both brighter and dimmer QI\_pts.  At a scale $R\approx500\kpchseventy$, brighter QI\_pt environments have an overdensity 1.6 times the overdensity of AI environments with significance $\approx3\sigma$, and dimmer QI\_pt environments have an overdensity 1.3 times the overdensity of AI environments with significance $\approx2\sigma$.  At $R\approx150\kpchseventy$, the environments of brighter QI\_pts are 2.1 times as overdense ($2.4\sigma$), and the environments of dimmer QI\_pts are 1.6 times as overdense as the environments of AIs ($2\sigma$).  

The ratio of QI\_pts to AIIs increases for both bright and dim quasars with decreasing scale, but less dramatically as the ratio to AIs.  The ratio between dimmer QI\_pts and AIIs is approximately consistent with unity for scales $150\kpchseventy\lesssim150\leq2.0\Mpchseventy$; the ratio between brighter QI\_pts and AIIs is 1.3 ($\gtrsim2\sigma$) for scales $R\gtrsim500\kpchseventy$.  On smaller scales, both ratios increase.  At scales $R\approx150\kpchseventy$, the ratio of brighter QI\_pts to AIIs is 1.6 ($\approx2\sigma$), and the ratio of dimmer QI\_pts to AIIs is 1.3 ($>1\sigma$).  This scale dependency could be evidence for the merger origin of quasars, since one would expect to see a higher density of environment galaxies at small scales where merger events are likely to take place \citep{Hopkins2008}. 

Evidence that dimmer quasars and lower-luminosity AGN are located in environments with similar overdensity might suggest that dimmer quasars could be a transition population between low-luminosity AGN (likely fueled in dry mergers, close encounters, or secular processes) and high-luminosity AGN (likely fueled in major mergers).  Rather than disparate populations of merger-fueled and secularly fueled AGN, there may be a continuum of galaxy interactions from major mergers to close encounters or harassment that cause AGN luminosity differences.  Alternatively, a mix of mergers and secular processes could drive the AGN population near the quasar-Seyfert divide \citep[$M_{i}\approx-22.5$;][]{Haob}.  We have compared the AGN samples without redshift cuts, but we note that in Section~\ref{redshiftsubsec} we demonstrated that evolution of quasar environments with redshift is negligible.  

The significant difference in the environments of bright QI\_pts and the environments of both AIs and AIIs could imply that these populations have different fueling mechanisms.  This result is consistent with results presented by \citet{Li2006, Li2008}, who find that there is only a weak link between nearby neighbors of narrow-line AGN and their nuclear activity.  

\section{BROAD-BAND LUMINOSITY, REDSHIFT, AND TYPE}\label{allsubsec}
We combine our analysis of type, redshift and absolute magnitude effects on environment overdensity in Figures~\ref{scale_spectargs_Mandz_higherz}, \ref{scale_spectargs_Mandz_lowerz}, and \ref{scale_qso_newMzcompare}.  Our $\delta z$ cuts on the photometric galaxies around the spectroscopic targets as well as around the random positions to which they are compared (as described in Section~\ref{deltazcutsection}) allow us to make meaningful comparisons of objects in different redshift ranges.  In Figure~\ref{scale_spectargs_Mandz_higherz}, QII\_Zs are compared to QI\_pts in the redshift range $0.3 \leq z \leq 0.6$.  
We divide the QI\_pts into bright ($2,001$; $\overline{M_{i}}=-23.87$) and dim ($1,915$; $\overline{M_{i}}=-22.75$, about 2.8 times fainter) samples of roughly equal numbers at $M_{i}=-23.25$.  

Comparing the lower panel of Figure~\ref{scale_spectargs_Mandz_higherz} to the top ratio panel of Figure~\ref{scale_spectargs_type} shows the dramatic part luminosity plays compared to evolution alone.  The environment of QII\_Zs is similar to the signature of brighter QI\_pts for all scales we measure.  The similarity of environments at small scales suggests that the differences observed between brighter Type I quasars and Type II quasars are due to a non-environmentally driven mechanism such as orientation or internal structure effects.  This in turn implies that Type II quasars are not a different cosmological population from these brighter Type I quasars.  

However, the QII\_Z environments are consistently more overdense, albeit with large errors, than those of dimmer QI\_pts on scales $R\leq2.0\Mpchseventy$ that we measure.  The different characteristics of the environments of the dimmer QI\_pt population from the QII\_Z population are most likely due to intrinsic luminosity differences rather than redshift differences.  
We see consistent overdensity ratios on all scales and do not see small scale effects, therefore we conclude that the difference in environment overdensity between the brighter and dimmer quasars is primarily due to mass effects.  More luminous AGN are expected to have higher mass black holes \citep[e.g.,][]{Magorrian, MarconiHunt}, which are in turn correlated with more massive dark matter halos \citep[e.g.,][]{FerrMerr, Gebhardt, Tremaine}.  
Selection effects in the magnitude-limited photometric galaxy sample could also play into the difference in overdensity between the brighter and dimmer QI\_pts.  The redshift distribution of QI\_pts in the brighter ($M_{i}\leq-23.25$) bin is slightly different from that of the dimmer ($M_{i}>-23.25$) bin even over the redshift range of $0.3 \leq z \leq 0.6$ (the brighter quasars have a mean redshift of 0.51, and the dimmer quasars have a mean redshift of 0.45).  The galaxies seen in the environments of brighter (higher redshift) quasars will tend themselves to be brighter, and consequently more massive, and therefore cluster more strongly than the dimmer environment galaxies \citep{Maddox, Zehavi}.  This, however, should not be a major effect.  

Figure~\ref{scale_spectargs_Mandz_lowerz} compares the environments of QI\_pts in two luminosity bins to the environments of AIs and AIIs in the redshift range $0.15<z\leq 0.33$.  We use $M_{i}=-22.65$ as the threshold value for brighter and dimmer quasars in this lower redshift range to equalize the number in each luminosity bin.  The $244$ brighter ($239$ dimmer) QI\_pts have a mean magnitude of  $\overline{M_{i}}=-22.33$ ($\overline{M_{i}}=-23.30$, about 2.4 times fainter than the brighter sample).  We note that these QI\_pt samples are about a factor of seven times smaller than the QI\_pt samples in the higher redshift range, thus the measurements (and resulting interpretation) will be less precise.  

The top panel of Figure~\ref{scale_spectargs_Mandz_lowerz} shows that at all scales, the environments of dimmer QI\_pts are more overdense than those of brighter QI\_pts.  It appears that the situation has been reversed from Figure~\ref{scale_spectargs_Mandz_higherz}, where the environments of dimmer quasars were less overdense than the environments of brighter quasars.  However, the range of luminosity at this lower redshift range of $0.15<z\leq0.33$ is much smaller than for the higher range of $0.3\leq z\leq 0.6$.  The overall absolute magnitude distribution of these QI\_pts is skewed toward the faint end, thus the dividing value $M_{i}=-22.65$ is very close to the quasar-Seyfert divide of $M_{i} \approx-22.5$ as defined by \citet{Haob}.   Significant variation in overdensities was seen when different magnitude cuts were imposed, with the dimmer quasars consistently having higher overdensities by varying margins.  The dramatic sensitivity of results on the bright/dim dividing value emphasize that for low luminosites and redshifts, broad-band absolute magnitudes are a poor proxy for AGN luminosity.  The measured flux is more likely to be affected by galaxy starlight, star formation, etc. at this faint end.  Therefore, any attempt to use broadband magnitudes to correlate nuclear luminosity with environment will be skewed.  

With these caveats in mind, we compare the QI\_pts to lower-luminosity AIs and AIIs in the lower two panels of the figure.  Dimmer QI\_pt environments have overdensities greater than the AIs, but the environments of brighter QI\_pts and the AIs have about the same amplitude on all scales.  The lower ratio panel shows the ratio of bright and dim QI\_pts to AIIs.  The brigher quasars have environments with slightly lower overdensity than AIIs;  the environments of dimmer QI\_pts are only slightly more overdense than the environments of AIIs, but are consistent within the error bars.  

In Figure~\ref{scale_qso_newMzcompare} we focus on QI\_pts alone to investigate the evolution of the environment overdensity of brighter and dimmer objects.   We have chosen two luminosity intervals of one magnitude in width and compare the environment overdensities of brighter to dimmer objects in three redshift intervals. $\Delta M_{1}$ corresponds to the dimmer luminosity interval of $-23.0<M_i\leq-22.0$ and contains 1,556 QI\_pts, and the brighter luminosity interval $\Delta M_2$ is $-24.0<M_{i}\leq-23.0$, containing 2,036 QI\_pts.  Table~\ref{table_Fig9Details} gives the number of quasars as well as the mean magnitude in each redshift and magnitude bin.  

In the two lower redshift bins $0.15<z\leq0.3$ and $0.3<z\leq0.45$, there is little difference in the environment overdensity of brighter and dimmer quasars with little-to-no scale dependence.  
However, in the highest redshift interval of $0.45 < z \leq 0.6$, brighter quasars are shown to be  located in slightly more overdense environments than the dimmer quasars.  At scale of $R\approx1.0\Mpchseventy$, the brighter quasars are located in environments with overdensity 1.5 times that of the dimmer quasars.  The brighter quasars have environments with overdensity 1.4 times the overdensity of dimmer quasar environments at a scale of $R\approx250\kpchseventy$, and then the ratio begins to drop toward unity at the innermost scales.  However, the large errors are nearly consistent with unity on all scales we measure.  

It appears, therefore, that there is again slight evidence for some redshift evolution of QI\_pt environments, but it is mainly manifested at the highest redshift range.  This emphasizes the need for additional studies of the environments around higher redshift Type I quasars.  We caution that the increased overdensity at higher redshift may be influenced by the fact that there are nearly three times the number of brighter quasars as dimmer quasars in the interval $0.45< z\leq0.6$ (see Table~\ref{table_Fig9Details}).  In the range $0.3<z\leq 0.45$, the number of bright quasars is closer to the number of dim quasars, while in the range $0.15<z\leq0.3$, the dim quasars outnumber the bright quasars by more than a factor of two.  The change in overdensity ratio will also be affected by the change in mean luminosity of the dimmer quasar sample with increasing redshift.  While the bright quasar luminosity changes only by 0.07 magnitudes, the mean dim quasar luminosity changes by 0.17 magnitudes.  Therefore we cannot draw strong conclusions, but reiterate the need for higher precision and higher redshift measurements of quasar environments.   

\begin{table}\centering \begin{minipage}{140mm}
\caption{Linear least-squared fit parameters for quasar environment data in Figure~\ref{redshift_spectargs}.  \label{table_compareFit}}
\begin{tabular}{c c c c c}\hline\hline
$R_{max}$&slope&intercept&$\chi^{2}$&P($\chi^{2}$,$\nu$)\\ \hline
$2.0\Mpchseventy$&0.119&-0.880&6.84&0.3363\\
&0.0&-0.833&8.10&0.3241\\
\cline{1-5}
$1.0\Mpchseventy$&0.140&-0.730&5.58&0.4719\\
&0.0&-0.677&6.04&0.5352\\
\cline{1-5}
$0.5\Mpchseventy$&0.691&-0.638&1.62&0.9514\\
&0.0&-0.388&4.17&0.7603\\
\cline{1-5}
$0.25\Mpchseventy$&1.276&-0.249&0.421&0.9987\\
&0.0&0.200&1.91&0.9646\\
\cline{1-5}
$0.1\Mpchseventy$&-1.171&2.066&0.628&0.9959\\
&0.0&1.635&0.716&0.9982
\end{tabular}
\end{minipage}
\end{table}

\begin{table}\centering \begin{minipage}{140mm}
\caption{Details for data used in Figure~\ref{scale_qso_newMzcompare}. \label{table_Fig9Details}}
\begin{tabular}{c c c}\hline\hline
Redshift Range&$-24.0<M_{i}\leq-23.0$&$-23.0<M_{i}\leq-22.0$\\ \hline
$0.15 < z \leq 0.3$& 85, $-23.39$&211, $-22.46$\\
$0.3 < z \leq 0.45$& 502, $-23.39$&788, $-22.57$\\
$0.45 < z \leq 0.6$& 1445, $-23.46$&552, $-22.63$
\end{tabular} \end{minipage}
\end{table}

\clearpage
\begin{figure}
\plotone{paper1figure2.pdf}
%\plotone{fig_scale_spectargcompare_HaoDR5_ptqso_nosplits_newminz_NOratio_newErr21jul.pdf}
\caption{Mean cumulative overdensity of photometric galaxies as a function of comoving scale around spectroscopic targets.  Solid black squares represent QI\_pts, open red starred points represent QII\_Zs, solid blue triangles represent AIIs, and solid green hexagons represent AIIs.   Points have been offset slightly for clarity.  
\label{scale_spectargs}}
\end{figure}

\begin{figure}
\plotone{paper1figure3.pdf}
\caption{Mean cumulative overdensity vs. redshift for spectroscopic targets.  Symbols correspond to those used in Figure~\ref{scale_spectargs}.  The magenta dashed lines are linear weighted least-squares fits for the QI\_pt sample; the parameters for these lines are given in Table~\ref{table_compareFit}.  
%\plotone{fig_redshift_spectargs_zevolfit_HaoDR5_ptqso_newminz_newErr21jul.pdf}
\label{redshift_spectargs}}
\end{figure}

\begin{figure}
\plotone{paper1figure4.pdf}
\caption{Upper panel:  Mean cumulative overdensity of photometric galaxies around quasars and lower-luminosity AGN as a function of scale and redshift.  Points have been offset slightly for clarity.  Top lower panel:  Ratio of environment overdensity of higher-redshift QI\_pts to that of lower-redshift QI\_pts.  Middle lower panel:   Ratio of environment overdensity of higher-redshift AIs to that of lower-redshift AIs.  Bottom lower panel:  Ratio of environment overdensity of higher-redshift AIIs to that of lower-redshift AIIs.    
%\plotone{fig_scale_spectargcompare_zsplit_zcompare_ptqso_newminz_newErr21jul.pdf}
\label{scale_spectargs_z}}
\end{figure}

\begin{figure}
\plotone{paper1figure5.pdf}
\caption{Upper panel:  Mean cumulative overdensity of photometric galaxies around quasars and lower-luminosity AGN as a function of scale and redshift.  Points have been offset slightly for clarity. Top lower panel:  Ratio of environment overdensity of QII\_Zs to that of QI\_pts in the redshift range $0.3 \leqslant z \leqslant 0.6$.  Middle lower panel:   Ratio of environment overdensity of AIIs to that of AIs in the redshift range $0.15 < z \leqslant 0.33$.  Bottom lower panel:  Ratio of environment overdensity of AIIs to that of AIs in the redshift range $0.11 < z \leqslant 0.15$.   
%\plotone{fig_scale_spectargcompare_zsplit_typecompare_ptqso_newminz_newErr21jul.pdf}
\label{scale_spectargs_type}}
\end{figure}

\begin{figure}
\plotone{paper1figure6.pdf}
\caption{Top panel:  Mean cumulative overdensity of photometric galaxies around QI\_pts split by luminosity; low luminosity AGN; and QII\_Zs.  Bright quasars have absolute magnitude $-27.5 \leq M_{i} \leq -23.2$ and dim quasars have absolute magnitude $-23.2 < M_{i} \leq -22.0$.  Top lower panel:  ratio of QII\_Zs environment overdensity to bright (solid points) and dim (open points) QI\_pt environment overdensities.  Middle lower panel:  ratio of bright (solid points) and dim (open points) QI\_pt environment overdensities to AI environment overdensity.  Bottom lower panel: ratio of bright (solid points) and dim (open points) QI\_pt environment overdensities to AII environment overdensity.  No redshift limits have been imposed.  
%\plotone{fig_scale_spectargcompare_Msplit_qsoptonly_HaoDR5_newminz_newErr21jul.pdf}
\label{scale_spectargs_M}}
\end{figure}

\begin{figure}
\plotone{paper1figure7.pdf}
\caption{Upper panel:  Mean cumulative overdensity of photometric galaxies around QII\_Zs and QI\_pts in the redshift range $0.3\leq z\leq0.6$.  The QI\_pts in this redshift range have been divided at $M_{i}=-23.25$ so that the luminosity bins contain approximately equal numbers of QI\_pts.  Lower panel:  Ratio of environment overdensities of QII\_Zs to brighter and dimmer QI\_pts in this redshift range.  Points in both panels have been offset slightly for clarity.  
%\plotone{fig_scale_spectargcompare_zsplit_higherz_newMsplit_ptqso_newErr21jul.pdf}
\label{scale_spectargs_Mandz_higherz}}
\end{figure}

\begin{figure}
\plotone{paper1figure8.pdf}
\caption{Upper panel:  Mean cumulative overdensity of photometric galaxies around QI\_pts and AIs and AIIs in the redshift range $0.15 < z \leq 0.33$.  The QI\_pts in this redshift range have been divided at $M_{i}=-22.65$ so that the luminosity bins contain approximately equal numbers of QI\_pts.  Lower panels:  Ratio of environment overdensities of brighter and dimmer QI\_pts to AIs and AIIs in this redshift range.  Points in both panels have been offset slightly for clarity.  
%\plotone{fig_scale_spectargcompare_zsplit_lowerz_newMsplit_ptqso_newErr21jul.pdf}
\label{scale_spectargs_Mandz_lowerz}}
\end{figure}

\begin{figure}
\plotone{paper1figure9.pdf}
\caption{Mean cumulative overdensity of photometric galaxies around QI\_pts with redshift for two luminosity bins, where $\Delta M_{1} : -23.0 < M_{i} \leq -22.0$ and $\Delta M_{2} : -24.0 < M_{i} \leq -23.0$.  Lower panels:  Ratio of $\Delta M_{2}$ to $\Delta M_{1}$ quasar environment overdensities in the three redshift ranges.  
%\plotone{fig_scale_ptqso_newMzcompare_zbins3_newminz_newErr21jul.pdf}
\label{scale_qso_newMzcompare}}
\end{figure}


%--------11z5 figures-----------
\clearpage
\begin{figure}
\plotone{paper1figure2_11z5.pdf}
\caption{Mean cumulative overdensity of photometric galaxies as a function of comoving scale around spectroscopic targets.  Solid black squares represent QI\_pts, open red starred points represent QII\_Zs, solid blue triangles represent AIIs, and solid green hexagons represent AIIs.   Points have been offset slightly for clarity.  
%dissfigs_paper1chapter_11z5.sm plotfig_scale_spectargcompare 1
\label{scale_spectargs}}
\end{figure}

\begin{figure}
\plotone{paper1figure3_11z5.pdf}
\caption{Mean cumulative overdensity vs. redshift for spectroscopic targets.  Symbols correspond to those used in Figure~\ref{scale_spectargs}.  The magenta dashed lines are linear weighted least-squares fits for the QI\_pt sample; the parameters for these lines are given in Table~\ref{table_compareFit}.  
%dissfigs_paper1chapter_11z5.sm plotfig_redshift_spectargs 1
\label{redshift_spectargs}}
\end{figure}

\begin{figure}
\plotone{paper1figure4_11z5.pdf}
\caption{Upper panel:  Mean cumulative overdensity of photometric galaxies around quasars and lower-luminosity AGN as a function of scale and redshift.  Points have been offset slightly for clarity.  Top lower panel:  Ratio of environment overdensity of higher-redshift QI\_pts to that of lower-redshift QI\_pts.  Middle lower panel:   Ratio of environment overdensity of higher-redshift AIs to that of lower-redshift AIs.  Bottom lower panel:  Ratio of environment overdensity of higher-redshift AIIs to that of lower-redshift AIIs.    
%dissfigs_paper1chapter_11z5.sm plotfig_scale_spectargcompare_zsplit 1
\label{scale_spectargs_z}}
\end{figure}

\begin{figure}
\plotone{paper1figure5_11z5.pdf}
\caption{Upper panel:  Mean cumulative overdensity of photometric galaxies around quasars and lower-luminosity AGN as a function of scale and redshift.  Points have been offset slightly for clarity. Top lower panel:  Ratio of environment overdensity of QII\_Zs to that of QI\_pts in the redshift range $0.3 \leqslant z \leqslant 0.5$.  Middle lower panel:   Ratio of environment overdensity of AIIs to that of AIs in the redshift range $0.15 < z \leqslant 0.33$.  Bottom lower panel:  Ratio of environment overdensity of AIIs to that of AIs in the redshift range $0.11 < z \leqslant 0.15$.   
%dissfigs_paper1chapter_11z5.sm plotfig_scale_spectargcompare_zsplit_typecompare 1
\label{scale_spectargs_type}}
\end{figure}

\begin{figure}
\plotone{paper1figure6_11z5.pdf}
\caption{Top panel:  Mean cumulative overdensity of photometric galaxies around QI\_pts split by luminosity; low luminosity AGN; and QII\_Zs.  Bright quasars have absolute magnitude $-26.4 \leq M_{i} \leq -23.0$ and dim quasars have absolute magnitude $-23.0 < M_{i} \leq -22.0$.  Top lower panel:  ratio of QII\_Zs environment overdensity to bright (solid points) and dim (open points) QI\_pt environment overdensities.  Middle lower panel:  ratio of bright (solid points) and dim (open points) QI\_pt environment overdensities to AI environment overdensity.  Bottom lower panel: ratio of bright (solid points) and dim (open points) QI\_pt environment overdensities to AII environment overdensity.  No redshift limits have been imposed.  
%dissfigs_paper1chapter_11z5.sm plotfig_scale_spectargcompare_lumsplit 1
\label{scale_spectargs_M}}
\end{figure}

\begin{figure}
\plotone{paper1figure7_11z5.pdf}
\caption{Upper panel:  Mean cumulative overdensity of photometric galaxies around QII\_Zs and QI\_pts in the redshift range $0.3\leq z\leq0.5$.  The QI\_pts in this redshift range have been divided at $M_{i}=-23.0$ so that the luminosity bins contain approximately equal numbers of QI\_pts.  Lower panel:  Ratio of environment overdensities of QII\_Zs to brighter and dimmer QI\_pts in this redshift range.  Points in both panels have been offset slightly for clarity.  
%dissfigs_paper1chapter_11z5.sm plotfig_scale_spectargcompare_higherz_eqMcut 1
\label{scale_spectargs_Mandz_higherz}}
\end{figure}

\begin{figure}
\plotone{paper1figure8_11z5.pdf}
\caption{Upper panel:  Mean cumulative overdensity of photometric galaxies around QI\_pts and AIs and AIIs in the redshift range $0.15 < z \leq 0.33$.  The QI\_pts in this redshift range have been divided at $M_{i}=-22.65$ so that the luminosity bins contain approximately equal numbers of QI\_pts.  Lower panels:  Ratio of environment overdensities of brighter and dimmer QI\_pts to AIs and AIIs in this redshift range.  Points in both panels have been offset slightly for clarity.  
%dissfigs_paper1chapter_11z5.sm plotfig_scale_spectargcompare_lowerz_eqMcut 1
\label{scale_spectargs_Mandz_lowerz}}
\end{figure}

\begin{figure}
\plotone{paper1figure9_11z5.pdf}
\caption{Mean cumulative overdensity of photometric galaxies around QI\_pts with redshift for two luminosity bins, where $\Delta M_{1} : -23.0 < M_{i} \leq -22.0$ and $\Delta M_{2} : -24.0 < M_{i} \leq -23.0$.  Lower panels:  Ratio of $\Delta M_{2}$ to $\Delta M_{1}$ quasar environment overdensities in the three redshift ranges.  
%dissfigs_paper1chapter_11z5.sm plotfig_scale_newMcompare_zbins3 1
\label{scale_qso_newMzcompare}}
\end{figure}

